Arbitrary Functors as Modalities in a Linear Calculus

We study modalities in the linear lambda calculus, by interpreting them as endofunctors in monoidal closed categories. We support functors that do not distribute over products, including (co)monads. We also support arbitrary natural transformations as conversion between modalities. We provide a generic categorical semantics, which we then specialise to a sound and complete resource semantics. We use this resource semantics to derive normalisation by evaluation. Along the way, we describe several applications of such models. This work aims at providing a foundation for future programming languages with modalities. The paper is backed by a mechanisation in Agda.

==> core_macros.tex <==

%%%%%%%%%%%
%% Contexts

\newcommand{\emptyContext}{[]}%{\mathbf{-}}
\newcommand\moda[1]{\prescript{#1}{}{\kern -1pt}}
% \newcommand\moda[1]{^{#1}}
\newcommand\Moda[1]{\text{\tikz[baseline=(X.base)]{\node(X)[draw,rounded corners=2,inner sep=2]{\ensuremath{#1}}}}}

%%%%%%%%%%%
%% Types And Terms

\newcommand\TBOX[2]{[^{#1} #2]}
\newcommand\BOX[1]{\Moda{#1}}
% \newcommand\BOX[2]{#1\langle#2\rangle}

\newcommand\funOp{⊸}
\NewDocumentCommand{\fun}{o m}{\IfNoValueTF{#1}{}{\BOX {#1}}#2 \funOp}
\NewDocumentCommand{\app}{o m}{\IfNoValueTF{#1}{\,#2}{\TBOX {#1}{#2}} }
\NewDocumentCommand{\lam}{o m}{λ\IfNoValueTF{#1}{#2}{\TBOX {#1}{#2}}. }

\newcommand\allM[1]{\forall #1.}
\newcommand\lamM[1]{\Lambda #1.}
\newcommand\appM[1]{\cdot #1}  % @@ looks ugly

\newcommand\Forall[1]{\forall #1.}
\newcommand\Lam[1]{\Lambda#1.}
\newcommand\App[1]{\cdot #1}  % @@ looks ugly

%% ⊗
\newcommand\Unit{1}
\newcommand\Tensor{⊗}

\newcommand\scase[6]{\mathsf{case}\, \moda {#1}#2\,\mathsf{of}\,\braces{\inl#3 \mapsto #4;\inr#5 \mapsto #6}}
\newcommand{\tinj}[1]{\mathsf{inj}_{#1}}

%% &
\newcommand{\With}{\mathbin{\&}}
\newcommand\twith[2]{⟨#1 , #2⟩}
\newcommand\ttop[1]{⟨⟩_{#1}}
\newcommand\Ttop{⊤}
\newcommand{\textr}[1]{\mathsf{proj}_{#1}}
\newcommand\tout[1]{\textr{#1}\,}

%% ⊕
\newcommand\Plus[3][]{#2 ⊕_{#1} #3}
\newcommand\tin[1]{\tinj{#1}\,}
\newcommand\inl{\tin1}%{\mathsf{inl}\,}
\newcommand\inr{\tin2}%{\mathsf{inr}\,}

%%%%%%%%%%%
%% Let and modality patterns

\newcommand\wlet[1]{\mathsf{let}\,#1\,\mathsf{in}\,}
\newcommand\ttlet{\mathsf{let}}
\newcommand\tlet[2]{\mathsf{let}\,#1=#2\,\mathsf{in}\,}
\newcommand\panalyse[4]{\ensuremath{\{\moda{#1} #2, \moda{#3} #4\}}}
% \newcommand\panalyse[2]{\ensuremath{[#1,#2]}}
% \newcommand\pthrow{\ensuremath{\mathsf{throw}}}
\newcommand\pthrow{\ensuremath{\{\}}}
% \newcommand\pthrow{\ensuremath{[]}}
% \newcommand\pconv[1]{\ensuremath{#1\,}} % looks too much like an application
% \newcommand\pconv[1]{\ensuremath{#1 ↦}}
\newcommand\pconv[2]{\ensuremath{#2 / #1}}

%%%%%%%%%%%%%
%% Side conditions

\newcommand\convertible{≼}

\newcommand\distributivity[1]{(∀ q r. pq + p r \convertible p(q + r) \convertible ∧ 0\convertible p0}
\newcommand\codistributivity[1]{∀ q r. p(q + r) \convertible pq + p r ∧ p0\convertible 0}
\newcommand\distributive{\ensuremath{δ}}
\newcommand\codistributive{\ensuremath{δ' }}
% \newcommand\caseable{ψ}
% \newcommand\isCaseable[1]{\ensuremath{#1 ∈ \caseable}}
\newcommand{\distributesMaybe}[2]{\ensuremath{(\lvert Γ \rvert = 1) ∨ \distributes{#2}}}
\newcommand\distributes[1]{\ensuremath{\distributive(#1)}}
\newcommand\codistributes[1]{\ensuremath{\codistributive(#1)}}
% \newcommand\distributes[1]{\ensuremath{#1 ∈ \distributive}}
% \newcommand\codistributes[1]{\ensuremath{#1 ∈ \codistributive}}


% Use |A| for carrier of A since A_c was confusing when c was used for sensitivity.
\newcommand{\carrier}[1]{\ensuremath{|#1|}}

%%%%%%%%%%%%%%%%%
% Rules

\newcommand\rul[1]{\ensuremath{\mbox{\normalfont\textsc{#1}}}}
\providecommand\rlet{\rul{let}}
\newcommand\BOXelim[1][p]{\ensuremath{\rul{\(\Moda {#1}\)-elim}}}
\newcommand\BOXintro[1][p]{\ensuremath{\rul{\({\Moda {#1}}\)-intro}}}

%%%%%%%%%%%%%%%%
%% Judgements
\providecommand\typatl[3]{\moda {#2} #3 ⊣ #1}
\providecommand\typat[4]{#2 : \moda {#3} #4 ⊣ #1}


%%%%%%%%%%%%%%%%%%%%%%
% Adjoints

\newcommand{\BOXin}[1][p]{\ensuremath{\BOX{#1}\mbox{-}{\overline{\rul{intro}}}}}
\newcommand{\BOXel}[1][p]{\ensuremath{\BOX{#1}\mbox{-}{\overline{\rul{elim}}}}}
\newcommand\tbox{\mathsf{box}}
\newcommand\tunbox{\mathsf{unbox}}
\newcommand\TBOXalt[1]{\ensuremath{\tbox^{#1}\,}}
\newcommand\TUNBOX[1]{\ensuremath{\tunbox^{#1}\,}}


==> macros.tex <==
\RequirePackage{ifthen}
%% NOT FOUND: \RequirePackage{mnsymbol} % \dotminus
%\RequirePackage{amssymb}
%\RequirePackage{amsfonts}
\RequirePackage{stmaryrd} % \shortuparrow

% evergreens
\newcommand{\bla}{\ensuremath{\mbox{$$}}} % invisible, but not ignored
\newcommand{\Fpure}{\ensuremath{\mathsf{F}}}
\newcommand{\Fomega}{\ensuremath{\mathsf{F}^\omega}}
\newcommand{\der}{\,\vdash}
\newcommand{\derP}{\der}%^+}
\newcommand{\of}{\!:\!}
\newcommand{\is}{\!=\!}
\newcommand{\sub}{\!\leq\!}
\newcommand{\red}{\longrightarrow}
\newcommand{\cored}{\longleftarrow}
\newcommand{\coredp}{\mathop{{}^+{\longleftarrow}}\nolimits}
\newcommand{\redbeta}{\red_\beta}
\newcommand{\redbetastar}{\red_\beta^*}
\newcommand{\coredbetastar}{\mathrel{\bla_\beta^*{\longleftarrow}}}
\newcommand{\redeta}{\red_\eta}
\newcommand{\expeta}{\red_{\eta^-}}
%\newcommand{\redbeta}{\mathrel{\red_\beta}}
%\newcommand{\redeta}{\mathrel{\red_\eta}}
%\newcommand{\coredeta}{\longleftarrow_\eta}
\newcommand{\redetastar}{\red_\eta^*}
\newcommand{\coredetastar}{\mathrel{\bla_\eta^*{\longleftarrow}}}
\newcommand{\redbetaeta}{\red_{\beta\eta}}
\newcommand{\redbetaetastar}{\red_{\beta\eta}^*}
\newcommand{\redw}{\mathrel{\red_{\mathsf{w}}}}
\newcommand{\whd}{\searrow} % for algorithmic equality
\newcommand{\rk}{\mathop{\mathsf{rk}}\nolimits}
\newcommand{\restrict}{\upharpoonright}
\newcommand{\isdef}{\downharpoonright}
\newcommand{\FV}{\ensuremath{\mathsf{FV}}}
\newcommand{\arity}{\ensuremath{\mathsf{ar}}}
%\newcommand{\otto}{\leftrightarrow} %contained in nath.sty
\newcommand{\Pot}{\mathcal{P}}
\newcommand{\dom}[1]{\mathsf{dom}(#1)}
\newcommand{\rng}{\mathop{\mathsf{rng}}\nolimits}
\newcommand{\pto}{\rightharpoonup} % partial map
\newcommand{\perto}{\stackrel{\mathsf{p}}\rightharpoonup} % partial coherent map
\newcommand{\pertot}{\stackrel{\mathsf{p}}\to} % coherent map
\newcommand{\kto}{\stackrel{\mathsf{K}}\rightharpoonup} % partial Kripke map
\newcommand{\NN}{\mathbb{N}}
\newcommand{\defas}{\mathrel{\ :\Longleftrightarrow\ }}
\newcommand{\defiff}{\mathrel{:\Longleftrightarrow}}
\newcommand{\substo}{\!\mapsto\!}
\newcommand{\mapstot}{\mathrel{\dot\mapsto}}
\newcommand{\condeq}{\doteq}
\newcommand{\aeq}{=_\alpha}
\newcommand{\beq}{=_{\beta}}
\newcommand{\beeq}{=_{\beta\eta}}
\newcommand{\enc}[1]{\ulcorner#1\urcorner}
%% for palatino
%\def\lv{\mathopen{[\kern-0.2em[}}    % opening [[ value delimiter
%\def\rv{\mathclose{]\kern-0.2em]}}   % closing ]] value delimiter
% for computer modern
\def\lv{\mathopen{{[\kern-0.14em[}}}    % opening [[ value delimiter
\def\rv{\mathclose{{]\kern-0.14em]}}}   % closing ]] value delimiter
\newcommand{\den}[1]{\lv #1 \rv}
\newcommand{\Den}[3][]{\den{#2}^{#1}_{#3}}
\newcommand{\dent}[2]{\llparenthesis#1\rrparenthesis_{#2}}
\newcommand{\dentcl}[1]{\llparenthesis#1\rrparenthesis}
  % banana brackets, need stmaryrd.sty
% for computer modern
% den in superscript
\newcommand{\dens}[1]{\mathopen{[\kern-0.3ex[}#1\mathclose{]\kern-0.3ex]}}
% kind interp.
\newcommand{\denk}[2]{\mathopen{\{\kern-0.3ex|}#1\mathclose{|\kern-0.3ex\}}_{#2}}
\newcommand{\length}[1]{\|#1\|}

% von Buchholz
\def\tox#1{\buildrel#1\over\to}
\def\ltox#1{\buildrel\raise1pt\hbox{$\scriptstyle#1$}\over\longrightarrow}
\def\toid{\tox{\scriptscriptstyle\rm id}}

\def\tocolow{\buildrel\raise-5pt\hbox{$\scriptscriptstyle+$}\over\rightarrow}

% \dotminus from http://tex.stackexchange.com/questions/114188/special-character-dot-over-dash
\makeatletter
\newcommand{\dotminus}{\mathbin{\text{\@dotminus}}}
\newcommand{\@dotminus}{%
  \ooalign{\hidewidth\raise1ex\hbox{.}\hidewidth\cr$\m@th-$\cr}%
}
\makeatother

% type equality
\def\lo{\mathopen{{\lceil\kern-0.25em\lceil}}}
\def\ro{\mathclose{{\rfloor\kern-0.25em\rfloor}}}
\newcommand{\ten}[1]{\lo#1\ro}
\newcommand{\Ten}[2]{\lo#1\ro_{#2}}
%\newcommand{\Tef}[2]{[#1]_{#2}}
\newcommand{\Tef}[2]{#1#2 \in \TYPE}
\newcommand{\Teq}[4]{#1#2 = #3#4 \in \TYPE}
%\newcommand{\Teq}[4]{\Tef{#1}{#2} = \Tef{#3}{#4}}

% normalization by evaluation
\newcommand{\twhnf}{\mathsf{whnf}}
\newcommand{\tnf}{\mathsf{nf}}
\newcommand{\nfraw}{\mathsf{nf}}
\newcommand{\nf}[3]{\nfraw(#1 \!\der\! #2 \!:\! #3)}
\newcommand{\nbe}[2]{\mathsf{nbe}_{#1}^{#2}}
\newcommand{\Nbe}[1]{\mathsf{Nbe}_{#1}}
\newcommand{\rhog}{\rho_\Gamma}
\newcommand{\rhogu}{\rho_{\cext\Gamma U}}
\newcommand{\rhogup}{\rho_{\cext\Gamma {U'}}}

% latin etc. abbrev
\newcommand{\abbrev}[1]{#1} % alternative: \emph{#1}
\newcommand{\cf}{\abbrev{cf.}\ }
\newcommand{\eg}{\abbrev{e.\,g.}}
\newcommand{\Eg}{\abbrev{E.\,g.}}
\newcommand{\ie}{\abbrev{i.\,e.}}
\newcommand{\Ie}{\abbrev{I.\,e.}}
\newcommand{\etal}{\abbrev{et.\,al.}}
\newcommand{\wwlog}{w.\,l.\,o.\,g.} % \wlog is ``write into log file''
\newcommand{\Wlog}{W.\,l.\,o.\,g.}
\newcommand{\wrt}{w.\,r.\,t.}

% paragraphs
\newcommand{\para}[1]{\paragraph*{\it#1}}
\newcommand{\paradot}[1]{\para{#1.}}

% proof by cases
\newenvironment{caselist}{%
  \begin{list}{{\it Case}}{%
    %\setlength{\topsep}{2ex}% DOES NOT SEEM TO WORK
    %\setlength{\itemsep}{2ex}%
    %\setlength{\itemindent}{-2ex}%
  }%
}{\end{list}%
}
\newenvironment{subcaselist}{%
  \begin{list}{{\it Subcase}}{}%
}{\end{list}%
}
\newenvironment{subsubcaselist}{%
  \begin{list}{{\it Subsubcase}}{}%
}{\end{list}%
}

\newcommand{\nextcase}{\item~}

% meta-level logic
\newcommand{\mfor}{\ \mbox{for}\ }
\newcommand{\mforsome}{\ \mbox{for some}\ }
\newcommand{\mthen}{\ \mbox{then}\ }
\newcommand{\mif}{\ \mbox{if}\ }
\newcommand{\miff}{\ \mbox{iff}\ }
\newcommand{\motherwise}{\ \mbox{otherwise}}
\newcommand{\mundefined}{\mbox{undefined}}
\newcommand{\mnot}{\mbox{not}\ }
\newcommand{\mand}{\ \mbox{and}\ }
\newcommand{\mor}{\ \mbox{or}\ }
\newcommand{\mimplies}{\ \mbox{implies}\ }
\newcommand{\mimply}{\ \mbox{imply}\ }
\newcommand{\mforall}{\ \mbox{for all}\ }
\newcommand{\mexists}{\mbox{exists}\ }
\newcommand{\mexist}{\mbox{exist}\ }
\newcommand{\mtrue}{\mbox{true}}
\newcommand{\mwith}{\ \mbox{with}\ }
\newcommand{\mwhere}{\ \mbox{where}\ }
\newcommand{\mholds}{\ \mbox{holds}\ }
\newcommand{\munless}{\ \mbox{unless}\ }
\newcommand{\mboth}{\ \mbox{both}\ }
\newcommand{\msuchthat}{\ \mbox{such that}\ }
% proofs
\newcommand{\msince}{\mbox{since}\ }
\newcommand{\mdef}{\mbox{by def.}}
\newcommand{\mass}{\mbox{assumption}}
\newcommand{\mhyp}{\mbox{by hyp.}}
\newcommand{\mlemma}[1]{\mbox{by Lemma~#1}}
\newcommand{\mih}[1][]{\mbox{by ind.hyp.}#1}
\newcommand{\mgoal}[1][]{\mbox{goal\ifthenelse{\equal{#1}{}}{}{~#1}}}
\newcommand{\mby}[1]{\mbox{by #1}}
\newcommand{\minfrule}{\mbox{by inference rule}}


% Inference rules
\newcommand{\rulename}[1]{\ensuremath{\mbox{\sc#1}}}
\newcommand{\rul}[2]{\dfrac{\begin{array}[b]{@{}l@{}} #1 \end{array}}{#2}}
\newcommand{\ru}[2]{\dfrac{\begin{array}[b]{@{}c@{}} #1 \end{array}}{#2}}
\newcommand{\rux}[3]{\ru{#1}{#2}\ #3}
\newcommand{\nru}[3]{#1\ \ru{#2}{#3}}
\newcommand{\nrux}[4]{#1\ \ru{#2}{#3}\ #4}
\newcommand{\dstack}[2]{\begin{array}[b]{c}#1\\#2\end{array}}
\newcommand{\ndru}[4]{#1\ \ru{\dstack{#2}{#3}}{#4}}
\newcommand{\ndrux}[5]{#1\ \ru{\dstack{#2}{#3}}{#4}\ #5}
\newcommand{\lcol}[1]{\multicolumn{1}{@{}l@{}}{{#1}}}
\newcommand{\rcol}[1]{\multicolumn{1}{@{}r@{}}{{#1}}}

% Substitution and function update
% read ``\subst F X A'' as ``substitute F for X in A''
%\newcommand{\subst}[3]{#3[#2 := #1]}
%\newcommand{\subst}[3]{[#1/#2]#3}
\newcommand{\subst}[3]{#3[#1/#2]}
% read ``\update \theta X \G'' as update \theta at point X by \G
\newcommand{\update}[3]{#1[#2 \mapsto #3]}
%\newcommand{\update}[3]{#1,#2 \is #3}


% %% ---------- %< ----------
% \DeclareRobustCommand*{\MakeCapital}[1]{%
% \begingroup
% \def\i{I}\def\j{J}%
% \def\do##1##2{\let##1##2\do}%
% \expandafter\do\@uclclist\relax{\relax\@gobble}%
% \let\protect\@gobble
% \def\do##1{\def##1####1{{\protect##1####1}}\do}%
% \expandafter\do\@caplist\do\relax
% \let\protect\noexpand
% \def\t##1##2{{\protect\t##1##2}}%
% \def\IeC##1{{\protect##1}}% -> inputenc
% \def\@tabacckludge##1##2{{% -> inputenc
% \expandafter\protect\csname\string##1\endcsname##2}}%
% \ifnum\catcode`\"=\active % -> babel
% \lccode`\~=`\"%
% \lowercase{\def~##1{{\protect\"##1}}}%
% \fi
% \edef\@tempa{#1}%
% \expandafter\endgroup
% \expandafter\@capitalize\@tempa}

% \def\@caplist{\"\`\^\~\"\=\.\H\b\c\d\r\u\v}
% \def\@capitalize#1{\uppercase{#1}}
% %% ---------- %< ----------

% ICFP 2018 paper

% colored overline
% https://tex.stackexchange.com/questions/57070/how-to-color-over-underline-or-other-ways-to-highlight-substituted-expressions
\newcommand{\coverline}[2]{\colorlet{temp}{.}\color{#1}\overline{\color{temp}#2}\color{temp}}


% ordinary color
\newcommand{\ocol}[1]{\textcolor{black}{#1}}
\newcommand{\ocolor}{\color{black}}
\definecolor{DeepJungleGreen}{rgb}{0.0, 0.29, 0.29}
\definecolor{DarkSpringGreen}{rgb}{0.09, 0.45, 0.27}
\definecolor{ForestGreenTraditional}{rgb}{0.0, 0.27, 0.13}
\definecolor{GreenPigment}{rgb}{0.0, 0.65, 0.31}
\definecolor{CalPolyPomonaGreen}{rgb}{0.12, 0.3, 0.17}
\definecolor{CSSGreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{DarkCerulean}{rgb}{0.03, 0.27, 0.49}
\definecolor{DarkRaspberry}{rgb}{0.53, 0.15, 0.34}

\colorlet{DarkBlue}{MidnightBlue!80!black}
\definecolor{HanBlue}{rgb}{0.27, 0.42, 0.81}
\definecolor{FrenchBlue}{rgb}{0.0, 0.45, 0.73}
\definecolor{EgyptianBlue}{rgb}{0.06, 0.2, 0.65}

\colorlet{TyColor}{EgyptianBlue} % ok
%\colorlet{TyColor}{FrenchBlue} % too weak
%\colorlet{TyColor}{HanBlue} % too weak
%\colorlet{TyColor}{AgdaFunction} % too strong
%\colorlet{TyColor}{AgdaFunction} %!70!gray} % DarkBlue
\newcommand{\tycol}[1]{\textcolor{TyColor}{#1}}

\colorlet{TmColor}{BrickRed}
\newcommand{\tmcolor}{\color{TmColor}}
\newcommand{\tmcol}[1]{\textcolor{TmColor}{#1}}
\newcommand{\tmc}[1]{\ensuremath{\mathsf{\tmcol{#1}}}}
\renewcommand{\t}{\tmcol{t}}
\newcommand{\e}{\tmcol{e}}

\newcommand{\heapcol}{\tmcol}
\newcommand{\h}{\heapcol{h}}
\newcommand{\hone}{\heapcol{h_1}}
\newcommand{\htwo}{\heapcol{h_2}}
\newcommand{\hr}{\tmuse{\rho}}
\newcommand{\hrp}{\tmuse{\rho'}}
\newcommand{\hrho}{\h^{\hr}}
\newcommand{\hann}[2]{\heapcol{#1}^{\tmuse{#2}}}
\newcommand{\hannp}[2]{\hann{(#1)}{#2}}
\newcommand{\hempty}{\heapcol{\emptyset}}

\definecolor{SpiroDiscoBall}{rgb}{0.06, 0.75, 0.99}
\definecolor{DeepSkyBlue}{rgb}{0.0, 0.75, 1.0}
\definecolor{DodgerBlue}{rgb}{0.12, 0.56, 1.0}

\colorlet{TyUseColor}{DodgerBlue}
%\colorlet{TyUseColor}{DeepSkyBlue} % too light
%\colorlet{TyUseColor}{SpiroDiscoBall} % too light
%\colorlet{TyUseColor}{SkyBlue!80!black}
%\colorlet{TyUseColor}{SkyBlue} % too light
\newcommand{\tyuse}[1]{\textcolor{TyUseColor}{#1}}

\colorlet{TmUseColor}{AgdaKeyword}%{Orange}
\newcommand{\tmuse}[1]{\textcolor{TmUseColor}{#1}}
\newcommand{\gam}[1][]{\ensuremath{\tmuse{\gamma_{#1}}}}

% Contexts
%\colorlet{CxtColor}{AgdaModule}%{Sepia}
\colorlet{CxtColor}{Sepia}
\newcommand{\cxtcol}[1]{\textcolor{CxtColor}{#1}}
\newcommand{\Gam}{\cxtcol{\Gamma}}

% Heap types
\newcommand{\htycol}{\cxtcol}
\renewcommand{\H}{\htycol{H}}

% De Bruijn indices
\colorlet{DBColor}{Gray!50!black}
\newcommand{\dbcol}[1]{\textcolor{DBColor}{#1}}
\newcommand{\indcol}[1]{\textcolor{DBColor}{#1}}
\renewcommand{\i}{\indcol{i}}
\renewcommand{\j}{\indcol{j}}

% Named variables
%\colorlet{VarColor}{Blue!80!black}}
\colorlet{VarColor}{CxtColor}
%\colorlet{VarColor}{RawSienna!80!black}
\newcommand{\varcol}[1]{\textcolor{VarColor}{#1}}
\newcommand{\x}{\varcol{x}}
\newcommand{\y}{\varcol{y}}
\newcommand{\z}{\varcol{z}}

%\colorlet{QColor}{AgdaField}  %% Rougly RubineRed
\colorlet{QColor}{RubineRed}
\newcommand{\qcol}[1]{\textcolor{QColor}{#1}}

\newcommand{\p}{\qcol{p}}
\newcommand{\pp}{\qcol{p'}}
\newcommand{\q}{\qcol{q}}
\newcommand{\qp}{\qcol{q'}}
\let\originalr=\r
\renewcommand{\r}{\qcol{r}}
\newcommand{\rp}{\qcol{r'}}
\newcommand{\qzero}{\ensuremath{\qcol{0}}}
\newcommand{\qone}{\ensuremath{\qcol{1}}}
\newcommand{\qomega}{\ensuremath{\qcol{\omega}}}
\newcommand{\qinfty}{\ensuremath{\qcol{\infty}}}
\newcommand{\qplus}{\mathbin{\qcol{+}}}
\newcommand{\qtimes}{\mathbin{\qcol{\cdot}}}
\newcommand{\qmeet}{\mathbin{\qcol{\wedge}}}
\newcommand{\qunion}{\mathbin{\qcol{\cup}}}
\newcommand{\qleq}{\mathrel{\qcol{\leq}}}
\newcommand{\qbot}{\ensuremath{\qcol{\bot}}}
\newcommand{\qtop}{\ensuremath{\qcol{\top}}}
\newcommand{\qset}[1]{\qcol{\{}#1\qcol{\}}}
\newcommand{\qround}[1]{\coverline{QColor}{#1}}
\newcommand{\qmid}{\mathrel{\qcol{\mid}}}
\newcommand{\qgetwo}{\qcol{{\geq}2}}
\newcommand{\qgeone}{\qcol{{\geq}1}}
\newcommand{\qleone}{\qcol{{\leq}1}}
\newcommand{\Q}{\qcol{\mathsf{Q}}}

\newcommand{\usage}[1]{{\tmuse|}#1{\tmuse|}}
\newcommand{\varusage}[2]{\usage{#1}^{\varcol{#2}}}
\newcommand{\tmvarusage}[2]{\varusage{\tmcol{#1}}{#2}}
\newcommand{\tmusage}[1]{\usage{\tmcol{#1}}}
\newcommand{\juse}[2]{\tmuse{#1}\tri\tmcol{#2}}

% Style-independent
\newcommand{\scext}[3]{\cxtcol{#1},\,\varcol{#2} : \tycol{#3}}
\newcommand{\ssub}[2]{\tycol{#1 \leq #2}}
\newcommand{\osingcxt}[3]{\tmcol{#1} :_{\qcol{#2}} \tycol{#3}} % old singleton context
\newcommand{\jty}[3]{\ensuremath{\cxtcol{#1} \der \tmcol{#2} : \tycol{#3}}}
\newcommand{\jisty}[2]{\ensuremath{\cxtcol{#1} \der \tycol{#2} : \Type}}

\newcommand{\eqrel}[1]{\stackrel{\qcol{#1}}{=}}

%\def\TRIANGLESTYLE{}

\ifdefined\TRIANGLESTYLE

\newcommand{\sty}[4]{\ensuremath{\cxtcol{#1} \der \tmuse{#2} \tri \tmcol{#3} : \tycol{#4}}}
\newcommand{\styp}[4]{\sty{#1}{#2}{#3}{#4}}

\newcommand{\cext}[4]{\cxtcol{#1},\,\tmcol{#2} : \tyuse{#3}{\tri}\tycol{#4}}
\newcommand{\wfty}[3]{\ensuremath{\cxtcol{#1} \der \tyuse{#2} \tri \tycol{#3}}}
\newcommand{\wty}[5]{\cxtcol{#1} \der \tmuse{#2} \tri \tmcol{#3} : \tyuse{#4} \tri \tycol{#5}}
\newcommand{\wtyp}[5]{\cxtcol{#1} \der \tmuse{#2} \tri \tmcol{#3} :
  \tyuse{#4} \tri \tycol{#5}}
\newcommand{\wtypl}{\wty}
\newcommand{\wtypr}{\wty}
%\newcommand{\wfvar}[4]{\tmcol{#2} : \tyuse{#3} \tri #4 \in \cxtcol{#1}}
\newcommand{\wfvar}[4]{\cxtcol{#1}(\tmcol{#2}) = \tyuse{#3} \tri \tycol{#4}}
\newcommand{\welim}[9]{\cxtcol{#1} \mid \tmuse{#2} \tri \tmcol{#3} :
  \tyuse{#4} \tri \tycol{#5} \der \tmuse{#6} \tri \tmcol{#7} :
  \tyuse{#8} \tri \tycol{#9}}
\newcommand{\welimpll}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\welimplr}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\welimprl}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\welimplrrl}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\welimpr}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\wsub}[4]{\cxtcol{#1} \der \tyuse{#2} \tri \tycol{#3} \leq \tycol{#4}}
\newcommand{\wsubp}[4]{\wsub{#1}{#2}{#3}{#4}}
\newcommand{\weq}[6]{\cxtcol{#1} \der \tmuse{#2} \tri \tmcol{#3} =
  \tmcol{#4} : \tyuse{#5} \tri \tycol{#6}}
% TODO: elimination equality \welq
\newcommand{\weqp}{\weq}
\newcommand{\weqpt}{\weq}
\newcommand{\weqpl}{\weq}
\newcommand{\weqplr}{\weq}
\newcommand{\weqplt}{\weq}
\newcommand{\wh}[3]{\tmuse{#2} \tri \heapcol{#1} : \cxtcol{#3}}

\else

\newcommand{\sty}[4]{\ensuremath{\cxtcol{#1} \der \tmcol{#3}^{\tmuse{#2}} : \tycol{#4}}}
\newcommand{\styp}[4]{\sty{#1}{#2}{(#3)}{#4}}

\newcommand{\cext}[4]{\cxtcol{#1},\,\tmcol{#2}{:}\tycol{#4}^{\tyuse{#3}}}
\newcommand{\wfty}[3]{\ensuremath{\cxtcol{#1} \der \tycol{#3}^{\tyuse{#2}}}}
\newcommand{\wty}[5]{\ensuremath{\cxtcol{#1} \der \tmcol{#3}^{\tmuse{#2}} : \tycol{#5}^{\tyuse{#4}}}}
\newcommand{\wtypl}[5]{\wty{#1}{#2}{(#3)}{#4}{#5}}
\newcommand{\wtypr}[5]{\wty{#1}{#2}{#3}{#4}{(#5)}}
\newcommand{\wtyp}[5]{\wty{#1}{#2}{(#3)}{#4}{(#5)}}
\newcommand{\wfvar}[4]{\cxtcol{#1}(\tmcol{#2}) = \tycol{#4}^{\tyuse{#3}}}
\newcommand{\welim}[9]{\cxtcol{#1} \mid \tmcol{#3}^{\tmuse{#2}}  :
  \tycol{#5}^{\tyuse{#4}} \der \tmcol{#7}^{\tmuse{#6}}  :
  \tycol{#9}^{\tyuse{#8}}}
\newcommand{\welimpll}[9]{\welim{#1}{#2}{(#3)}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\welimplr}[9]{\welim{#1}{#2}{#3}{#4}{(#5)}{#6}{#7}{#8}{#9}}
\newcommand{\welimprl}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{(#7)}{#8}{#9}}
\newcommand{\welimplrrl}[9]{\welim{#1}{#2}{#3}{#4}{(#5)}{#6}{(#7)}{#8}{#9}}
\newcommand{\welimpr}[9]{\welim{#1}{#2}{#3}{#4}{#5}{#6}{(#7)}{#8}{(#9)}}
\newcommand{\wsub}[4]{\cxtcol{#1} \der \tycol{#3}^{\tyuse{#2}} \leq \tycol{#4}^{\tyuse{#2}}}
\newcommand{\wsubp}[4]{\wsub{#1}{#2}{(#3)}{(#4)}}
\newcommand{\weq}[6]{\cxtcol{#1} \der \tmcol{#3}^{\tmuse{#2}} =
  \tmcol{#4}^{\tmuse{#2}} : \tycol{#6}^{\tyuse{#5}}}
\newcommand{\weqp}[6]{\weq{#1}{#2}{(#3)}{(#4)}{#5}{(#6)}}
\newcommand{\weqpl}[6]{\weq{#1}{#2}{(#3)}{#4}{#5}{#6}}
\newcommand{\weqplr}[6]{\weq{#1}{#2}{(#3)}{(#4)}{#5}{#6}}
\newcommand{\weqplt}[6]{\weq{#1}{#2}{(#3)}{#4}{#5}{(#6)}}
\newcommand{\weqpt}[6]{\weq{#1}{#2}{#3}{#4}{#5}{(#6)}}
\newcommand{\wh}[3]{\heapcol{#1}^{\tmuse{#2}} : \cxtcol{#3}}

\fi
\newcommand{\ABSSIDE}{} % Side condition for abstraction

\newcommand{\REMOVEUSAGE}{%
\renewcommand{\sty}[4]{\ensuremath{\cxtcol{##1} \der \tmcol{##3} : \tycol{##4}}}%
\renewcommand{\styp}[4]{\sty{##1}{##2}{##3}{##4}}%
%
\renewcommand{\cext}[4]{\cxtcol{##1},\,\tmcol{##2}{:}\tycol{##4}}%
\renewcommand{\wfty}[3]{\ensuremath{\cxtcol{##1} \der \tycol{##3}}}%
\renewcommand{\wty}[5]{\ensuremath{\cxtcol{##1} \der \tmcol{##3} : \tycol{##5}}}%
\renewcommand{\wtypl}[5]{\wty{##1}{##2}{##3}{##4}{##5}}%
\renewcommand{\wtypr}[5]{\wty{##1}{##2}{##3}{##4}{##5}}%
\renewcommand{\wtyp}[5]{\wty{##1}{##2}{##3}{##4}{##5}}%
\renewcommand{\wfvar}[4]{\cxtcol{##1}(\tmcol{##2}) = \tycol{##4}}%
\renewcommand{\welim}[9]{\cxtcol{##1} \mid \tmcol{##3}  : \tycol{##5} \der \tmcol{##7}  : \tycol{##9}}%
\renewcommand{\welimpll}[9]{\welim{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
\renewcommand{\welimplr}[9]{\welim{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
\renewcommand{\welimprl}[9]{\welim{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
\renewcommand{\welimplrrl}[9]{\welim{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
\renewcommand{\welimpr}[9]{\welim{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
\renewcommand{\wsub}[4]{\cxtcol{##1} \der \tycol{##3} \leq \tycol{##4}}%
\renewcommand{\wsubp}[4]{\wsub{##1}{##2}{##3}{##4}}%
\renewcommand{\weq}[6]{\cxtcol{##1} \der \tmcol{##3} = \tmcol{##4} : \tycol{##6}}%
\renewcommand{\weqp}[6]{\weq{##1}{##2}{##3}{##4}{##5}{##6}}%
\renewcommand{\weqpl}[6]{\weq{##1}{##2}{##3}{##4}{##5}{##6}}%
\renewcommand{\weqplr}[6]{\weq{##1}{##2}{##3}{##4}{##5}{##6}}%
\renewcommand{\weqplt}[6]{\weq{##1}{##2}{##3}{##4}{##5}{##6}}%
\renewcommand{\weqpt}[6]{\weq{##1}{##2}{##3}{##4}{##5}{##6}}%
%
\renewcommand{\wh}[3]{\heapcol{##1} : \cxtcol{##3}}%
\renewcommand{\ABSSIDE}{\q \qleq \tmvarusage t x}
} % END REMOVE USAGE

\newcommand{\wcxt}[1]{\ensuremath{\der \cxtcol{#1}}}
\newcommand{\whcxt}{\wcxt}
\newcommand{\tri}{\triangleright}
%\newcommand{\oneuse}[1]{#1^1}
\newcommand{\oneuse}[1]{#1{:}\qone}
\newcommand{\zerouse}[1]{#1{:}\qzero}
\newcommand{\zerooneuse}[1]{#1{:}\qcol{\{0,1\}}}
\newcommand{\nouse}{\emptyset}
\newcommand{\snouse}{\tmuse{\emptyset}}
\newcommand{\suext}[3]{\ensuremath{\tmuse{#1},\varcol{#2}{:}{\qcol{#3}}}}
\newcommand{\uext}[3]{\ensuremath{#1,#2{:}#3}}
\newcommand{\umul}[2]{#1#2}
\newcommand{\uunion}[2]{#1 \cup #2}
\newcommand{\tmuunion}[2]{\tmuse{#1 \cup #2}}
\newcommand{\open}[2]{#1[#2]}
\newcommand{\apply}[3]{#1\cdot^{#2}#3}
\newcommand{\sapply}[3]{\tmcol{#1}\cdot^{\qcol{#2}}\tmcol{#3}}
\newcommand{\ann}[2]{{}^{#1}#2}
\newcommand{\annp}[2]{{}^{#1}(#2)}

\newcommand{\eempty}{\varepsilon}

% reduction
\newcommand{\whr}{\red_{\mathsf{w}}}
\newcommand{\hwr}{\cored_{\mathsf{w}}}
\newcommand{\whe}{\searrow}
\newcommand{\hwe}{\swarrow}
\newcommand{\whred}[2]{\tmcol{#1} \whr \tmcol{#2}}
\newcommand{\wheval}[2]{\tmcol{#1} \evalsto \tmcol{#2}}
\newcommand{\contr}{\mapsto}
\newcommand{\contract}[2]{\tmcol{#1} \contr \tmcol{#2}}

% colonized judgements
\newcommand{\colonize}[1]{\mathrel{{:}{#1}{:}}}
\newcommand{\cwhr}{\colonize{\whr}}
\newcommand{\chwr}{\colonize{\hwr}}
\newcommand{\cwhe}{\colonize{\whe}}
\newcommand{\chwe}{\colonize{\hwe}}
\newcommand{\ceq}{\colonize{=}}
\newcommand{\cweq}[6]{\cxtcol{#1} \der^{\tmuse{#2}} \tmcol{#3} \ceq \tmcol{#4} : \tycol{#6}^{\tyuse{#5}}}
\newcommand{\cwheval}[6]{\cxtcol{#1} \der^{\tmuse{#2}} \tmcol{#3} \cwhe \tmcol{#4} : \tycol{#6}^{\tyuse{#5}}}

% proof terms
\newcommand{\prfN}[2]{\underline{\mathcal{N}}(\tycol{#1},\tycol{#2})}

% logical relation
\newcommand{\LRT}[5]{\cxtcol{#1} \Vdash^{\tyuse{#2}} \tycol{#3} = \tycol{#4} : \Univ{#5}}
\newcommand{\LRD}[7]{\cxtcol{#1} \Vdash^{\tmuse{#2}} \tmcol{#3} = \tmcol{#4} : \tycol{#6}^{\tyuse{#5}} /_{#7}}

\newcommand{\simsubst}[2]{#1[#2]}
\newcommand{\opar}[1]{\ocol{(}#1\ocol{)}}
\newcommand{\hden}[2]{\heapcol{#1}^*\opar{\tmcol{#2}}}
\newcommand{\hiter}[3]{\heapcol{#1}^*_{\varcol{#2}}\opar{\tmcol{#3}}}
\newcommand{\hiteralign}[2]{\heapcol{#1}^*_{\varcol{#2}}}
\newcommand{\sgh}[2]{\heapcol{\{#1 \mapsto #2\}}}
\newcommand{\DAG}[1]{\heapcol{#1}\;\mathsf{dag}}

% Machines
\newcommand{\mstate}[4]{\heapcol{#1}^{\tmuse{#2}} \Vdash \tmcol{#3} \app \tmcol{#4}}


% ICFP 2017 paper

% Intro

\newcommand{\vpre}{\mathit{pre}}
\newcommand{\vpost}{\mathit{post}}
\newcommand{\ttrav}{\mathsf{trav}}
\newcommand{\tof}{\tmc{of}}
\newcommand{\vts}{\mathit{ts}}
\newcommand{\tnode}{\mathsf{node}}
\newcommand{\One}{\mathbf{1}}

\newcommand{\Size}{\mathsf{Size}}
\newcommand{\SizeExp}{\mathsf{SizeExp}}
\newcommand{\Data}{\mathsf{Data}}
\newcommand{\FixK}{\mathsf{FixK}}
\newcommand{\FixT}{\mathsf{FixT}}

\newcommand{\piSizeT}[1]{\Pi\,\Size\,#1\,}
\newcommand{\forallT}{\forall\,}

\newcommand{\tsuc}{\tmc{suc}}
\newcommand{\tcase}{\tmc{case}}
\newcommand{\tfix}{\mathsf{fix}}

\newcommand{\suc}[1]{\tmcol{\tsuc\,#1}}
\newcommand{\fix}[2][]{\tfix_{#1}\,#2\,}
\newcommand{\case}[6]{\tcase^{#1,#2}_{#3,#4}\,#5\,#6}

\newcommand{\caseqrlc}{\case q r \ell C}
\newcommand{\fixtt}{\fix[\ell] T t}

\newcommand{\eeq}{\risingdotseq}
\newcommand{\suty}[4]{#1 \der #2 \eeq #3 : #4}
\newcommand{\sueq}[5]{#1 \der #2 = #3 \eeq #4 : #5}

\newcommand{\sqsubsetsim}{\mathrel{\substack{\scriptstyle\sqsubset\\[-0.6ex]\scriptstyle\sim}}}
%\newcommand{\sqsubsetsim}{\mathrel{\substack{\textstyle\sqsubset\\[-0.2ex]\textstyle\sim}}}
\newcommand{\shape}{\sqsubsetsim}
\newcommand{\ssh}[4]{#1 \valid #2 \shape #3 /_{#4}}

\newcommand{\The}{\Theta}

%\newcommand{\Rty}[3]{\mathop{\mathsf{R}}\nolimits^{\mathsf{ty}}_{#1} \, #2 \evalsto #3}
\newcommand{\Rty}[3]{\mathsf{R}^{\mathsf{ty}}_{#1} \, #2 \evalsto #3}
\newcommand{\RTy}[3]{\mathsf{R}^{\mathsf{ty}}_{#1} \, #2 \evalsto #3}
\newcommand{\RUp}[3]{\mathsf{R}^{\mathsf{up}}_{#1} \, #2 \evalsto #3}
\newcommand{\RNe}[3]{\mathsf{R}^{\mathsf{ne}}_{#1} \, #2 \evalsto #3}
\newcommand{\RNat}[3]{\mathsf{R}^{\mathsf{nat}}_{#1} \, #2 \evalsto #3}
\newcommand{\RSize}[3]{\mathsf{R}^{\mathsf{size}}_{#1} \, #2 \evalsto #3}
\newcommand{\RElim}[3]{\mathsf{R}^{\mathsf{elim}}_{#1} \, #2 \evalsto #3}
\newcommand{\R}[3]{\mathsf{R}_{#1} \, #2 \evalsto #3}
\newcommand{\tRne}{\mathsf{R}^{\mathsf{ne}}}
\newcommand{\tRsize}{\mathsf{R}^{\mathsf{size}}}
\newcommand{\tRty}{\mathsf{R}^{\mathsf{ty}}}
\newcommand{\tRelim}{\mathsf{R}^{\mathsf{elim}}}
\newcommand{\tR}{\mathsf{R}}

\newcommand{\monus}{\dotminus} %{\stackrel{\cdot}{-}}
\newcommand{\Adm}{\mathsf{Adm}\,}
\newcommand{\nfeq}{\approx}
%\newcommand{\nfeq}{\equiv}
\newcommand{\asub}{\mathrel{{<}{:}}}

% % natural transformations
% \newcommand{\subscriptopt}[1]{\ifthenelse{\equal{#1}{}}{}{_{#1}}}
% \newcommand{\superscriptopt}[1]{\ifthenelse{\equal{#1}{}}{}{^{#1}}}
% \newcommand{\nattrans}[1][]{\Rightarrow\superscriptopt{#1}}

% % semantical inclusion and saturated sets
% \newcommand{\lsub}[1][]{\sqsubseteq\superscriptopt{#1}}
% \newcommand{\lsuper}[1][]{\sqsupseteq\superscriptopt{#1}}
% \newcommand{\lsup}[1][]{\textstyle\bigsqcup\superscriptopt{#1}}
% \newcommand{\linf}[1][]{\textstyle\bigsqcap\superscriptopt{#1}}
% \newcommand{\lcup}[1][]{\textstyle\sqcup\superscriptopt{#1}}
% \newcommand{\lcap}[1][]{\textstyle\sqcap\superscriptopt{#1}}
% \newcommand{\lbot}[1][]{\textstyle\bot\superscriptopt{#1}}
% \newcommand{\ltop}[1][]{\textstyle\top\superscriptopt{#1}}

% relational model
\newcommand{\uPi}[2][\,]{\underline\Pi^{#1}#2\,}
\newcommand{\PP}{\mathsf{PP}}

% polarities
\newcommand{\Pol}{\mathsf{Pol}}
\newcommand{\pmixed}{\mathord{\circ}}%{\mathord{\cdot}} %{\mathord{\pm}}
\newcommand{\pco}{\mathord{+}}
\newcommand{\pcontra}{\mathord{-}}
\newcommand{\pin}{\mathord{\bullet}}%{\top}%{\mathord{0}}
\newcommand{\pinv}[1]{#1^{-1}}

% Universe Polymorphism
\newcommand{\Level}{\mathsf{Level}}
\newcommand{\lzero}{0}
\newcommand{\lsucc}{\mathop{1\mathord+}}
\newcommand{\linfty}{\omega}
\newcommand{\eq}[1][]{\stackrel{#1}{=}}
\newcommand{\eqm}{\eq[m]}
\newcommand{\shapecheck}{\mathord{\ominus}}
\newcommand{\eqs}{\eq[\shapecheck]}
\newcommand{\resm}{\resurrect[m]}
\newcommand{\resmef}{\resm{\evarof}}

\newcommand{\wfcxt}[1]{\der\resurrect{#1}}
\newcommand{\eqcxt}[2]{\mathord{\wfcxt{#1}} \eqs \mathord{\wfcxt{#2}}}
\newcommand{\sheqty}[4]{\mathord{\wfty{#1}{#2}} \eqs \mathord{\wfty{#3}{#4}}}
\newcommand{\Seto}{\Set\linfty}

%equality and typing
\newcommand{\Erel}[1]{\mathrel{:\mathrel{#1}:}}
%\newcommand{\E}{\Erel{=}}
\newcommand{\Ecum}{\Erel{\cum}}
\newcommand{\Ecocum}{\Erel{\cocum}}

\newcommand{\Acum}{\trianglelefteq}
\newcommand{\Acumcl}{\closerel{\trianglelefteq}}
\newcommand{\Acocum}{\trianglerighteq}
\newcommand{\Acocumcl}{\closerel{\trianglerighteq}}

% TYPES 2010 paper
\newcommand{\squashtype}[1]{|\!|#1|\!|}
\newcommand{\sqval}[1]{[#1]}
\newcommand{\tsquash}{\sqval{\_}} %{\mathsf{squash}}
\newcommand{\tsqelim}{\mathsf{sqelim}}
\newcommand{\subT}[3]{\{ #1 : #2 \mid #3 \}}
\newcommand{\Composite}{\mathsf{Composite}}

% INRIA 2011 talk
%\newcommand{\sem}[3]{\mathsf{sem}(#1 \der #2^{#3})}
% \newcommand{\tm}[2]{\mathsf{tm}(#1 \der #2)}
% \newcommand{\enf}[2]{\overline{\mathsf{eq}}(#1 \der #2)}
% \newcommand{\ene}[2]{\underline{\mathsf{eq}}(#1 \der #2)}
\newcommand{\sem}[3][]{\mathsf{sem}(#2)_{#1}^{#3}}
\newcommand{\tm}[2]{\mathsf{tm}(#2)_{#1}}
\newcommand{\enf}[2]{\overline{\mathsf{eq}}(#2)_{#1}}
\newcommand{\ene}[2]{\underline{\mathsf{eq}}(#2)_{#1}}
\newcommand{\sort}[1]{\mathsf{sort}(#1)}
\newcommand{\KPer}[1]{\mathsf{KPer}(#1)}
\newcommand{\pnf}[3][]{\overline{#2}_{#1}^{#3}}
\newcommand{\pne}[3][]{\underline{#2}_{#1}^{#3}}

% FoSSaCS 2011 paper
\newcommand{\close}[1]{\widehat{#1}}

% long version
\newcommand{\squash}[1]{#1^{\div}}
%\newcommand{\R}{\mathrel{\circledR}}
%\newcommand{\Rcl}{\R}%{\mathrel{\widehat{\circledR}}}
%\newcommand{\Univ}[1]{\mathcal{U}\kern-0.3ex\mathit{niv}_{#1}}
\newcommand{\Univ}[1]{\mathsf{U}_{#1}}
\newcommand{\ePIAF}{\Pi^{\evar}\,\A\,\F}
\newcommand{\erPIAF}{\Pi^{\div}\,\A\,\F}
\newcommand{\eA}{\A^{\evar}}

% sigma types
\newcommand{\epairT}[4][\evar]{(#2#1#3) \times #4}
\newcommand{\erpairT}{\epairT[\erased]}
\newcommand{\pairT}{\epairT[\!:\!]}
\newcommand{\wpairT}{\epairT[:]} % wide colon
\newcommand{\letin}[4]{\tlet~(#1,#2) = #3 ~\tin~ #4}

% weak head normalization
\newcommand{\eappa}[1][\evar]{\,@^{#1}\,}
\newcommand{\erappa}{\eappa[\erased]}
\newcommand{\nerappa}{\eappa[:]}
\newcommand{\appa}{\eappa[]}

% algorithmic equality
\newcommand{\whnf}[1]{\mathord{\downarrow}#1}
\newcommand{\eqinfr}{\longleftrightarrow}
\newcommand{\eqchkr}{\Longleftrightarrow}
\newcommand{\eqinf}{\mathrel{\eqinfr}}
\newcommand{\eqchk}{\mathrel{\eqchkr}}
\newcommand{\eqty}{\eqchk}
\newcommand{\eqlvl}{\eqinf}
\newcommand{\eqinftr}{\mathrel{\mbox{$\kern1.7ex\widehat{}\kern-2.6ex\longleftrightarrow$}}}
\newcommand{\eqchktr}{\mathrel{\mbox{$\kern1.7ex\widehat{}\kern-2.6ex\Longleftrightarrow$}}}
\newcommand{\eqinft}{\mathrel{\eqinftr}}
\newcommand{\eqchkt}{\mathrel{\eqchktr}}
\newcommand{\eqtyt}{\eqchkt}
%\newcommand{\eqinft}{~\buildrel\cdot\over\longleftrightarrow~}
%\newcommand{\eqchkt}{~\buildrel\cdot\over\Longleftrightarrow~}
\newcommand{\EqNat}[3]{#1 \der #2 \eqchk #3 : \tNat}

% PTS
\newcommand{\Axiom}{\mathsf{Axiom}}
\newcommand{\Rule}{\mathsf{Rule}}
\newcommand{\EPTS}{\textrm{EPTS}\xspace}

% examples
\newcommand{\tok}{\mathsf{ok}}
\newcommand{\tT}{\mathsf{T}}
% Leibniz eq
\newcommand{\tsym}{\mathsf{sym}}
\newcommand{\tsubst}{\mathsf{subst}}
% semi groups
\newcommand{\vassoc}{\mathit{assoc}}
\newcommand{\Assoc}{\mathsf{Assoc}}
\newcommand{\SemiGrp}{\mathsf{SemiGrp}}
\newcommand{\tflip}{\mathsf{flip}}
\newcommand{\tthm}{\mathsf{thm}}


% Heterogeneous model
\newcommand{\nA}{A}
\newcommand{\nB}{B}
\newcommand{\ldom}[1]{{#1}^{\tL}}
\newcommand{\rdom}[1]{{#1}^{\tR}}
\newcommand{\inv}[1]{{#1}^{-1}}
\newcommand{\lr}[1]{\overrightarrow{#1}}
\newcommand{\rl}[1]{\overleftarrow{#1}}
%\newcommand{\smash}[1]{\lfloor#1\rfloor}

% DTP talk
\newcommand{\texI}{\mathsf{exI}}
\newcommand{\tsubI}{\mathsf{subI}}
\newcommand{\tmap}{\mathsf{map}}


% JFLA talk
\newcommand{\ttunit}{\mathtt{unit}}
\newcommand{\tttt}{\mathtt{tt}}
\newcommand{\ttEmptyset}{\mathtt{Empty\_set}}
\newcommand{\tteq}{\mathtt{eq}}
\newcommand{\tteqrect}{\mathtt{eq\_rect}}
\newcommand{\ttreflequal}{\mathtt{refl\_equal}}
\newcommand{\ttvector}{\mathtt{vector}}
\newcommand{\ttVcons}{\mathtt{Vcons}}
\newcommand{\ttVhead}{\mathtt{Vhead}}
\newcommand{\ttVtail}{\mathtt{Vtail}}
\newcommand{\ttS}{\mathtt{S}}
\newcommand{\ttnat}{\mathtt{nat}}
\newcommand{\ttType}{\mathtt{Type}}
\newcommand{\ttSet}{\mathtt{Set}}
\newcommand{\ttunitrect}{\mathtt{unit\_rect}}
\newcommand{\ttInductive}{\mathtt{Inductive}}
\newcommand{\ttProd}{\mathtt{Prod}}
\newcommand{\ttfst} {\mathtt{fst}}
\newcommand{\ttsnd} {\mathtt{snd}}
\newcommand{\ttpair}{\mathtt{pair}}
\newcommand{\ttBla}{\mathtt{Bla}}
\newcommand{\ttfoo}{\mathtt{foo}}
\newcommand{\ttbar}{\mathtt{bar}}
\newcommand{\ttbool}{\mathtt{bool}}
\newcommand{\tttrue}{\mathtt{true}}
\newcommand{\ttfalse}{\mathtt{false}}
\newcommand{\ttSized}{\mathtt{Sized}}
\newcommand{\ttSize}{\mathtt{Size}}
\newcommand{\ttProp}{\mathtt{Prop}}
\newcommand{\ttO}{\mathtt{O}}
\newcommand{\ttAcc}{\mathtt{Acc}}


% Awodey-Bauer where
\newcommand{\ABwhere}[3]{#1 \; \mathsf{where}\; [#2] \leftarrow #3}
\newcommand{\MYwhere}[3]{#1 \; \mathsf{where}\; #2 \leftarrow #3}
\newcommand{\tlet}{\mathsf{let}}
\newcommand{\tin}{\mathsf{in}}

% MPC/LiCS 10 paper
\newcommand{\IITT}{\textrm{IITT}\xspace}
\newcommand{\ICC}{\textrm{ICC}\xspace}
\newcommand{\ICCstar}{\textrm{ICC}\ensuremath{^*}\xspace}
\newcommand{\derI}{\der_{\ICCstar}}
\newcommand{\ICCh}{\textrm{ICC}\ensuremath{^\mathrm{h}}\xspace}
\newcommand{\funF}[2]{\piT{#2}}
\newcommand{\sig}{\Sigma}
\newcommand{\erasepar}[1]{(#1)^*}
\newcommand{\erhyp}{\!\div\!}
\newcommand{\erof}{\div}
% mathabx
\newcommand{\nsof}{\mathrel{\overline:}}% {\mathrel{:\kern-1.3ex\mbox{-}}}% {\divdot} % \odiv % \boxdiv %AMS: \therefore
%txfonts/pxfonts: \coloneq :- % \maya{3}
\newcommand{\nonstrict}{\mathord{\nsof}}
\newcommand{\nsext}{\erext[\nonstrict]}
\newcommand{\evar}{\mathord{\star}}
\newcommand{\evarof}{\star}
\newcommand{\erased}{\mathord{\div}}
\newcommand{\noterased}{\mathord{:}}
\newcommand{\eside}{\evar \in \{\erased,\noterased\}}
\newcommand{\eann}[1]{\erann[\evar]{#1}}
\newcommand{\erann}[2][\erased]{{}^{#1}#2}%{#2^{#1}}
\newcommand{\csep}{\ .\ }
\newcommand{\erext}[3][\erased]{\cext{#2}\erann[#1]{#3}}
\newcommand{\eext}[2]{\erext[\evar]{#1}{#2}}
\newcommand{\erlam}[2]{\lambda [#1 \of #2].\,}
\newcommand{\erapp}[2]{#1[#2]}
\newcommand{\vbla}{\mathit{bla}}
\newcommand{\tnil}{\mathsf{nil}}
\newcommand{\tcons}{\mathsf{cons}}
\newcommand{\vas}{\mathit{as}}
\newcommand{\tlength}{\mathsf{length}}
\newcommand{\tlookup}{\mathsf{lookup}}
\newcommand{\String}{\mathsf{String}}
\newcommand{\tVec}{\mathsf{Vec}}
\newcommand{\Fin}{\mathsf{Fin}}
\newcommand{\tfzero}{\mathsf{fzero}}
\newcommand{\tfsuc}{\mathsf{fsuc}}
\newcommand{\tabort}{\mathsf{abort}}
\newcommand{\abort}[1]{\tabort_{#1\,}}
\newcommand{\tunit}{\langle\rangle}%{()}
\newcommand{\Natrec}{\mathsf{Natrec}}
\newcommand{\tnatrec}{\mathsf{natrec}}
\newcommand{\natrec}[3]{\tnatrec_{#1\,}#2\,#3\,}
\newcommand{\erpiT}[2][\erased]{\Pi\erann[#1]{#2}\,}%{\Pi\,\erann[#1]{#2}\,}
\newcommand{\erfunT}[3][\erased]{\Pi#2#1#3.\,}%{\Pi\,\erann[#1]{#2}\,}
\newcommand{\epiT}[1]{\erpiT[\evar]{#1}}
\newcommand{\alT}[1]{\forall\,#1\,}
\newcommand{\alD}[2]{\forall#1 \!\in\! #2.\;}
\newcommand{\piD}[2]{\Pi#1 \!\in\! #2.\;}
\newcommand{\epiD}[2]{\epiT #1 \!\in\! #2.\;}
\newcommand{\Set}[1][]{\tSet_{#1}}
\newcommand{\dersig}{\der_\Sigma}
\newcommand{\derpsig}{\der_{(\Sigma)}}
\newcommand{\dero}{\der^o}
\newcommand{\derop}{\der^{o'}}
\newcommand{\derc}{\der^\tc}
\newcommand{\dera}{\der^\ta}
\newcommand{\deri}{\der^\ti}
%\newcommand{\tc}{\mathsf{c}}
\newcommand{\ta}{\mathsf{a}}
\newcommand{\ti}{\mathsf{i}}
\newcommand{\bracket}[2][]{[#2]^{#1}}
\newcommand{\envle}{\preccurlyeq}
%\newcommand{\close}[1]{\overline{#1}}
\newcommand{\Denc}[2]{\close{\llbracket{#1}\rrbracket}_{#2}}

% FLOPS 10 paper
\newcommand{\piT}{\PiT}
\newcommand{\piV}[1]{\underline\Pi\,#1\,}
\newcommand{\lm}[1]{\lambda\,#1\,}
\newcommand{\pidot}[1]{\Pi\,#1.\,}
\newcommand{\pivdot}[1]{\underline\Pi\,#1.\,}
\newcommand{\lmdot}[1]{\lambda\,#1.\,}
\newcommand{\Abs}{\mathsf{Abs}}

% explicit substitutions
\newcommand{\sempty}{()}
\newcommand{\sext}[2]{(#1,#2)}
\newcommand{\sid}{\mathsf{id}}
\newcommand{\scomp}[1]{#1\,}
\newcommand{\slift}{\mathord{\shortuparrow}}
\newcommand{\sg}[1]{[#1]}
\newcommand{\esubst}[1]{#1\,}
%\renewcommand{\inst}[2]{#1{\sg{#2}}}
%\renewcommand{\inst}[2]{\esubst{#1}{\sg{#2}}}
\newcommand{\lift}[1]{\esubst{#1}\slift}
\newcommand{\clm}[1]{\underline\lambda #1}
\newcommand{\clos}[1]{(\underline\lambda #1)}
% closure forming (instead of \dent)
\newcommand{\clost}[2]{\esubst{#1}{#2}}
\newcommand{\closp}[2]{\esubst{(#1)}{#2}}
\newcommand{\clostp}[2]{\esubst{#1}{(#2)}}
\newcommand{\clospp}[2]{\esubst{(#1)}{(#2)}}
% new stuff for Kripke-Relations
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\krel}[4]{#1 \der #2 \sim #3 \in #4}
\newcommand{\kabs}[2]{#1.#2}
\newcommand{\kall}[1]{\bigcap #1}
\newcommand{\kne}[1]{\underline{#1}}
\newcommand{\knf}[1]{\overline{#1}}
\newcommand{\Knf}[1]{\overline{\overline{#1}}}
\newcommand{\karrowi}{\rulename{k-fun-i}}
\newcommand{\karrowe}{\rulename{k-fun-e}}
\newcommand{\kforalli}{\rulename{k-all-i}}
\newcommand{\kforalle}{\rulename{k-all-e}}
\newcommand{\real}[1][]{\Vdash^{#1}}
\newcommand{\ttype}{\mathord{*}}

% weak normalization
\newcommand{\eqclass}[1]{\overline{#1}}

\newcommand{\idenv}[1]{\sid_{#1}}
\newcommand{\eval}[2]{\dent{#2}{\idenv{#1}}}
\newcommand{\evall}[2]{\clost{#2}{\idenv{#1}}} % lazy
\newcommand{\evalsto}{\searrow}
\newcommand{\at}{\mathrel{@}}
\newcommand{\Eval}[2]{\dent{#1}{#2} \evalsto}
\newcommand{\EvalPar}[2]{\dent{#1}{#2} \evalsto}
% \newcommand{\Eval}[2]{#1\,#2 \evalsto}
% \newcommand{\EvalPar}[2]{(#1)\,#2 \evalsto}
% \newcommand{\App}[2]{#1 \dapp #2 \evalsto}
\newcommand{\Read}[2]{#1 \der #2 \evalsto}
\newcommand{\ReadNe}[2]{#1 \der^{\mathsf{ne}} #2 \evalsto}
\newcommand{\Rne}[1]{\mathsf{R}^{\mathsf{ne}}_{#1}\,}
\newcommand{\Rnf}[1]{\mathsf{R}^{\mathsf{nf}}_{#1}\,}
% \newcommand{\Rne}[1]{\mathop{\mathsf{R}}\nolimits^{\mathsf{ne}}_{#1}}
% \newcommand{\Rnf}[1]{\mathop{\mathsf{R}}\nolimits^{\mathsf{nf}}_{#1}}
\newcommand{\Equal}[3]{#1 \der #2 \cong #3}
\newcommand{\Abstract}[4]{#1,#2 \der #3 \ltox{\lambda} #4}


% % Lambda-Pi-Nat-U constants
% \newcommand{\Fun}{\mathsf{Fun}}
\newcommand{\tN}{\mathsf{N}}
% \newcommand{\U}{\mathsf{U}}
\newcommand{\tz}{\mathsf{z}}
%\newcommand{\ts}{\mathsf{s}}
% \newcommand{\trec}{\mathsf{rec}} % primitive recursion
% \newcommand{\Rec}{\mathsf{Rec}} % type of primitive recursion


% semantics
\newcommand{\dlam}[2]{\mathsf{lam}^{#1}\,#2\,}
\newcommand{\dfun}[2]{\mathsf{fun}^{#1}\,#2\,}
\newcommand{\app}[2]{#1\cdot#2}

\newcommand{\funS}[2]{(#1 : #2) \to}
\newcommand{\allS}[2]{\forall #1 : #2.}
\newcommand{\sigT}[2]{\Sigma #1 \of #2.\,}
\newcommand{\funT}[2]{(#1 \of #2) \to}
\newcommand{\sfunT}[2]{(#1 : #2) \to}
\newcommand{\allT}[2]{\forall #1 \of #2. \,}
%\newcommand{\allT}[2]{[#1 \of #2] \to}

\newcommand{\knet}[3]{\kne{#1,#2 \reifiesto #3}}
\newcommand{\knft}[3]{\knf{#1,#2 \reifiesto #3}}
%\newcommand{\Rbase}[5]{#1 : #2 \reifiesto #3 \der #4 : #5}
%\newcommand{\Rne}[4]{#1 \der #2 \reifiesto #3 : #4}

\newcommand{\tString}{\tycol{\mathsf{String}}}
\newcommand{\Bool}{\tycol{\mathsf{Bool}}}
\newcommand{\tBool}{\tycol{\mathsf{Bool}}}
\newcommand{\Nat}{\tycol{\mathsf{Nat}}}
\newcommand{\tNat}{\tycol{\mathsf{Nat}}}
\newcommand{\tzero}{\tmc{zero}}

\newcommand{\Rec}[4]{\mathsf{Rec}^{#1}(#2,#3,#4)}
\newcommand{\trec}{\mathsf{rec}}
\newcommand{\rec}[4]{\trec^{#1}(#2,#3,#4)}

\renewcommand{\AA}{\mathfrak{A}}
\newcommand{\FF}{\mathfrak{F}}

\newcommand{\erase}[1]{|#1|}
\newcommand{\KiCand}[1]{\langle\!\langle #1 \rangle\!\rangle}%{\mathsf{Cand}(#1)}
\newcommand{\Cand}[1]{\langle #1 \rangle}%{\mathsf{Cand}(#1)}
\newcommand{\PiC}[2][\,]{\Pi^{#1}#2\,}
\newcommand{\PiK}[2][\,]{\Pi^{#1}#2\,}
\newcommand{\PIK}[2][]{\prod\nolimits^{#1}#2\,}
\newcommand{\AllC}[1]{\forall\,#1\,}
\newcommand{\PiChat}[1]{\hat\Pi\,#1\,}
\newcommand{\PiKhat}[2][\,]{\hat\Pi^{#1}#2\,}
\newcommand{\PIKhat}[2][]{\mathop{\hat\prod}\nolimits^{#1}#2\,}
\newcommand{\AllChat}[1]{\hat\forall\,#1\,}
\newcommand{\Forall}[2][\,]{\forall^{#1}#2\,}
\newcommand{\Forallhat}[1]{\hat\forall\,{#1}\,}
\newcommand{\FunChat}[1]{\hat{\mathsf{\lambda}}^{#1}\,}
\newcommand{\FunKhat}[1]{\dot{\mathsf{\lambda}}^{#1}\,}
\newcommand{\Funhat}[1]{\hat{\mathsf{\lambda}}^{#1}}
%\newcommand{\U}{\mathcal{U}}
\newcommand{\uu}{\mathcal{u}}
\newcommand{\acal}{\mathcal{a}}
\newcommand{\bb}{\mathcal{b}}
\newcommand{\tcal}{\mathcal{t}}

%\newcommand{\Bot}[1]{\bot^{#1}}
%\newcommand{\Top}[1]{\top^{#1}}
\newcommand{\inter}{\mathrel{\wedge}}
\newcommand{\Inter}[1]{\bigcap^{#1}}
\newcommand{\tdom}{\diamond}%\circ
\newcommand{\ttm}{\tdom}

\newcommand{\SimpleKind}{\mathsf{SimpleKind}}
\newcommand{\SKi}{\mathsf{SKi}}
\newcommand{\SKiP}{\mathsf{SKiP}}
\newcommand{\SCxt}{\mathsf{SCxt}}
\newcommand{\haskind}{\div}
\newcommand{\hasskel}{\doteq}
\newcommand{\haskindo}{\mathord{\haskind}}
\newcommand{\hasskelo}{\mathord{\hasskel}}
\newcommand{\staro}{\mathord{\star}}
\newcommand{\shapeof}[3][]{|#2|^{#1}_{#3}}
\newcommand{\kindof}{\shapeof[\haskindo]}
\newcommand{\skelof}{\shapeof[\hasskelo]}
\newcommand{\kindsub}{\shapeof[]}%\kindof is too crowded
\newcommand{\skelcxt}[1]{|#1|}

\newcommand{\resurrecttwice}[1]{#1^{\mathord{\oplus}\mathord{\oplus}}}
\newcommand{\resurrect}[2][]{#2^{\ifthenelse{\equal{#1}{}}{\oplus}{%\overline{
#1}}}%}
\newcommand{\eresurrect}[1]{\resurrect[\evar]{#1}}
\newcommand{\erresurrect}{\resurrect[\div]}
\newcommand{\nsresurrect}{\resurrect[\nonstrict]}


\newcommand{\To}{\Rightarrow}

% macros for composing syntax
\newcommand{\sarr}[3]{\tycol{#2} \tox{\qcol{#1}} \tycol{#3}}
\newcommand{\arr}[3]{#2 \tox{#1} #3}
%\newcommand{\arr}[3]{#2 \mathrel{{}^{#1}{\to}} #3}
\newcommand{\PiT}[4]{\Pi^{#1,#2}#3\,#4}
\newcommand{\FunT}[3]{\Fun\,#2\,\lambda#1 #3}%{\Fun\,#2\,(\lambda#1.#3)}
\newcommand{\FunV}[2]{\Fun\,#1\,#2}
\newcommand{\succT}[1]{\ts\,#1}
\newcommand{\recT}[1][]{\trec\,(#1)} %{\trec_{#1}}
\newcommand{\RecT}[1][]{\Rec\,(#1)} %{\Rec_{#1}}
\newcommand{\lam}[1]{\lambda^{#1}\,}
\newcommand{\nlam}[2]{\lambda^{#2} #1.\,}
\newcommand{\snlam}[2]{\lambda^{\qcol{#2}}\varcol{#1}.\,}
%\newcommand{\nlam}[2]{\lambda #1^{#2}.\,}
\newcommand{\lamdot}[1]{\lambda^{#1}.\,}

\newcommand{\Id}[3]{\mathsf{Id}_{#1}\,#2\,#3}
\newcommand{\trefl}{\mathsf{refl}}
\newcommand{\tidElim}{\mathsf{idElim}}
\newcommand{\idElim}[6]{\tidElim_{#1,#2,#3}\,#4\,#5\,#6}
\newcommand{\tirr}{\mathord{*}}
\newcommand{\tcomp}{\mathsf{comp}}

\newcommand{\tif}{\tmc{if}}
\newcommand{\tifzero}{\tmc{ifzero}}
\newcommand{\tthen}{\tmc{then}}
\newcommand{\telse}{\tmc{else}}
\newcommand{\tifthenelse}[3]{\tif\,#1\,\tthen\,#2\,\telse\,#3}
\newcommand{\ifzero}[3]{\tifzero\,#1\,\tthen\,#2\,\telse\,#3}
%\newcommand{\tifthenelse}[3]{\tif\;#1\;\tthen\;#2\;\telse\;#3}

% LFSigma legacy
\newcommand{\Pair}{\mathsf{Pair}}
\newcommand{\tREL}[1][]{\mathcal{R}\!\mathit{el}_{#1}}
\newcommand{\REL}[2][]{\tREL[#1](#2)}
% \newcommand{\REL}[3][]{\tREL[#1](#2,#3)}
\newcommand{\tEl}[1][]{\mathcal{E}\!\mathit{l}_{#1}}
\newcommand{\El}[2][]{\tEl[#1](#2)}
\newcommand{\ElNoPar}[1][]{\tEl[#1]}
\newcommand{\tSet}{\mathsf{Set}}
\newcommand{\Type}[1][]{\mathsf{Type}_{#1}}
\newcommand{\Prop}{\mathsf{Prop}}

% syntactic classes
\newcommand{\Quant}{\mathsf{Quant}}
\newcommand{\Sort}{\mathsf{Sort}}
\newcommand{\tkind}{\Box}
\newcommand{\Ty}{\mathsf{Ty}}
\newcommand{\Exp}{\mathsf{Exp}}
\newcommand{\Ann}{\mathsf{Ann}}
\newcommand{\LamII}{\Lambda^{\downarrow\uparrow}}
\newcommand{\Kind}{\mathsf{Kind}}
\newcommand{\Ki}{\mathsf{Ki}}
\newcommand{\Constr}{\mathsf{Constr}}
\newcommand{\Obj}{\mathsf{Obj}}
\newcommand{\Elim}{\mathsf{Elim}}
\newcommand{\Atom}{\mathsf{Atom}}
\newcommand{\Const}{\mathsf{Const}}
\newcommand{\Proj}{\mathsf{Proj}}
\newcommand{\Par}{\mathsf{Par}}
\newcommand{\Clos}{\mathsf{Clos}}
\newcommand{\Cxt}{\mathsf{Cxt}}
\newcommand{\WCxt}{\mathsf{WCxt}}
\newcommand{\WNe}{\mathsf{WNe}}
\newcommand{\Wne}{\mathsf{Wne}}
\newcommand{\Whnf}{\mathsf{Whnf}}
\newcommand{\Wbase}{\mathsf{Wbase}}
\newcommand{\WVal}{\mathsf{WVal}}
\newcommand{\WFun}{\mathsf{WFun}}
\newcommand{\WPair}{\mathsf{WPair}}
\newcommand{\WElim}{\mathsf{WElim}}
\newcommand{\Env}{\mathsf{Env}}
\newcommand{\Tm}{\mathsf{Tm}}
\newcommand{\BVar}{\mathsf{BVar}}
\newcommand{\FVar}{\mathsf{FVar}}
\newcommand{\Var}{\mathsf{Var}}
\newcommand{\Ne}{\mathsf{Ne}}
\newcommand{\NeExp}{\mathsf{NeExp}}
\newcommand{\Null}{\emptyset}
\newcommand{\Unit}{()}
\newcommand{\NeUnit}{\Ne^{()}}
\newcommand{\DNe}{\mathsf{DNe}}
\newcommand{\Nf}{\mathsf{Nf}}
\newcommand{\DNf}{\mathsf{DNf}}
\newcommand{\Neut}{\mathsf{Neut}}
\newcommand{\Norm}{\mathsf{Norm}}
\newcommand{\VNe}{\mathsf{VNe}}
\newcommand{\Val}{\mathsf{Val}}
\newcommand{\VFun}{\mathsf{VFun}}
\newcommand{\VPair}{\mathsf{VPair}}
\newcommand{\FVal}{\mathsf{FVal}}
\newcommand{\PVal}{\mathsf{PVal}}
\newcommand{\GVal}{\mathsf{GVal}}
\newcommand{\tfst}{\mathsf{fst}}
\newcommand{\tsnd}{\mathsf{snd}}
\newcommand{\tS}{\mathsf{S}}
\newcommand{\tK}{\mathsf{K}}
\newcommand{\tI}{\mathsf{I}}


% rules for the lambda-model
\newcommand{\rvar}{\rulename{var}}
\newcommand{\rapp}{\rulename{app}}
\newcommand{\rcase}{\rulename{case}}
\newcommand{\rarg}{\rulename{arg}}
\newcommand{\rapptwo}{\rulename{app2}}
\newcommand{\rabs}{\rulename{abs}}
\newcommand{\rzero}{\rulename{zero}}
\newcommand{\rsuc}{\rulename{suc}}
\newcommand{\rifzero}{\rulename{ifzero}}
\newcommand{\reta}{\rulename{eta}}
\newcommand{\rcontr}{\rulename{contr}}
\newcommand{\rbeta}{\rulename{beta}}
\newcommand{\rbetam}{\rulename{beta$^{-}$}}
\newcommand{\retam}{\rulename{eta$^{-}$}}
\newcommand{\rirr}{\rulename{irr}}
\newcommand{\rsubst}{\rulename{subst}}
\newcommand{\rbetap}{\rulename{beta$^{+}$}}
\newcommand{\rxi}{\rulename{xi}}
\newcommand{\rext}{\rulename{ext}}
\newcommand{\rleqeta}{\rulename{leq-eta}}
\newcommand{\rleqapp}{\rulename{leq-app}}
\newcommand{\rS}{\rulename{S}}
\newcommand{\rK}{\rulename{K}}


% context rules
\newcommand{\ok}{}%{\mathsf{ok}}
\newcommand{\cxtpref}{cxt-}
\newcommand{\rcxtempty}{\rulename{\cxtpref{}empty}}
\newcommand{\rcxtext}{\rulename{\cxtpref{}ext}}

% rules for substitutions
\newcommand{\substpref}{subst-}
\newcommand{\rsubstempty}{\rulename{\substpref{}empty}}
\newcommand{\rsubstext}{\rulename{\substpref{}ext}}
\newcommand{\eqsubstpref}{\eqpref{}\substpref{}}
\newcommand{\reqsubstempty}{\rulename{\eqsubstpref{}empty}}
\newcommand{\reqsubstext}{\rulename{\eqsubstpref{}ext}}

% semantical context
\newcommand{\semcxtpref}{sem-cxt-}
\newcommand{\rsemcxtempty}{\rulename{\semcxtpref{}empty}}
\newcommand{\rsemcxtext}{\rulename{\semcxtpref{}ext}}

% typing rule names
\newcommand{\typref}{}%{ty-}
\newcommand{\natpref}{n-}%{nat-}
\newcommand{\rhyp}{\rulename{\typref{}hyp}}
\newcommand{\rconst}{\rulename{\typref{}const}}
\newcommand{\rconv}{\rulename{\typref{}conv}}
%\newcommand{\rsubst}{\rulename{\typref{}subst}}
\newcommand{\rpi}{\rulename{\typref{}pi}}
\newcommand{\runiv}{\rulename{\typref{}univ}}
\newcommand{\ruf}{\rulename{\typref{}univ-f}}
\newcommand{\ruin}{\rulename{\typref{}univ-i-n}}
\newcommand{\ruifun}{\rulename{\typref{}univ-i-fun}}
\newcommand{\rue}{\rulename{\typref{}univ-e}}
\newcommand{\rsetf}{\ruf}%{\rulename{\typref{}set-f}}
\newcommand{\rsete}{\rue}%{\rulename{\typref{}set-e}}
\newcommand{\rfunf}{\rulename{\typref{}fun-f}}
\newcommand{\rpairf}{\rulename{\typref{}pair-f}}
\newcommand{\rfuni}{\rulename{\typref{}fun-i}}
\newcommand{\rfune}{\rulename{\typref{}fun-e}}
\newcommand{\rpairi}{\rulename{\typref{}pair-i}}
\newcommand{\rpairel}{\rulename{\typref{}pair-e-l}}
\newcommand{\rpairer}{\rulename{\typref{}pair-e-r}}
\newcommand{\rnatf}{\rulename{\typref{}\natpref{}f}}
\newcommand{\rnatiz}{\rulename{\typref{}\natpref{}i-z}}
\newcommand{\rnatis}{\rulename{\typref{}\natpref{}i-s}}
\newcommand{\rnate}{\rulename{\typref{}\natpref{}e}}


% equality rule names
\newcommand{\eqpref}{eq-}
\newcommand{\reqsig}{\rulename{\eqpref{}$\Sigma$}}
\newcommand{\reqeta}{\rulename{\eqpref{}$\eta$}}
\newcommand{\reqbeta}{\rulename{\eqpref{}$\beta$}}
\newcommand{\reqfun}{\rulename{\eqpref{}fun}}
\newcommand{\reqvar}{\rulename{\eqpref{}var}}
\newcommand{\reqlam}{\rulename{\eqpref{}lam}}
\newcommand{\reqapp}{\rulename{\eqpref{}app}}
\newcommand{\reqerapp}{\rulename{\eqpref{}[app]}}
\newcommand{\reqsort}{\rulename{\eqpref{}sort}}
\newcommand{\reqrefl}{\rulename{\eqpref{}refl}}
\newcommand{\reqsym}{\rulename{\eqpref{}sym}}
\newcommand{\reqtrans}{\rulename{\eqpref{}trans}}
\newcommand{\reqreflty}{\rulename{\eqpref{}refl-ty}}
\newcommand{\reqsymty}{\rulename{\eqpref{}sym-ty}}
\newcommand{\reqtransty}{\rulename{\eqpref{}trans-ty}}
\newcommand{\reqconst}{\rulename{\eqpref{}const}}
\newcommand{\reqhyp}{\rulename{\eqpref{}hyp}}
\newcommand{\reqsubst}{\rulename{\eqpref{}subst}}
\newcommand{\reqconv}{\rulename{\eqpref{}conv}}
\newcommand{\reqsetf}{\rulename{\eqpref{}univ-f}}
\newcommand{\reqsete}{\rulename{\eqpref{}univ-e}}
\newcommand{\reqfunf}{\rulename{\eqpref{}fun-f}}
\newcommand{\reqpairf}{\rulename{\eqpref{}pair-f}}
\newcommand{\reqfuni}{\rulename{\eqpref{}fun-i}}
\newcommand{\reqfune}{\rulename{\eqpref{}fun-e}}
\newcommand{\reqfunbeta}{\rulename{\eqpref{}fun-$\beta$}}
\newcommand{\reqfuneta}{\rulename{\eqpref{}fun-$\eta$}}
\newcommand{\reqpairi}{\rulename{\eqpref{}pair-i}}
\newcommand{\reqpairel}{\rulename{\eqpref{}pair-e-l}}
\newcommand{\reqpairer}{\rulename{\eqpref{}pair-e-r}}
\newcommand{\reqpairbetal}{\rulename{\eqpref{}pair-$\beta$-l}}
\newcommand{\reqpairbetar}{\rulename{\eqpref{}pair-$\beta$-r}}
\newcommand{\reqpaireta}{\rulename{\eqpref{}pair-$\eta$}}
\newcommand{\reqfunc}{\rulename{\eqpref{}func}}
\newcommand{\reqfuncty}{\rulename{\eqpref{}func-ty}}
\newcommand{\reqnatf}{\rulename{\eqpref{}\natpref{}f}}
\newcommand{\reqnatiz}{\rulename{\eqpref{}\natpref{}i-z}}
\newcommand{\reqnatis}{\rulename{\eqpref{}\natpref{}i-s}}
\newcommand{\reqnate}{\rulename{\eqpref{}\natpref{}e}}
\newcommand{\reqnatiotaz}{\rulename{\eqpref{}\natpref{}$\iota$-z}}
\newcommand{\reqnatiotas}{\rulename{\eqpref{}\natpref{}$\iota$-s}}


% evaluation
\newcommand{\evalpref}{eval-}
\newcommand{\revalid}{\rulename{\evalpref{}id}}
\newcommand{\revalc}{\rulename{\evalpref{}c}}
\newcommand{\revalatom}{\rulename{\evalpref{}atom}}
\newcommand{\revalvar}{\rulename{\evalpref{}var}}
\newcommand{\revale}{\rulename{\evalpref{}e}}
\newcommand{\revalfuni}{\rulename{\evalpref{}fun-i}}
\newcommand{\revalfune}{\rulename{\evalpref{}fun-e}}
\newcommand{\revalpairi}{\rulename{\evalpref{}pair-i}}
\newcommand{\revalpaire}{\rulename{\evalpref{}pair-e}}
\newcommand{\revalpairel}{\rulename{\evalpref{}pair-e-l}}
\newcommand{\revalpairer}{\rulename{\evalpref{}pair-e-r}}

% active elimination (was: application)
%\newcommand{\apppref}{app-}
\newcommand{\apppref}{elim-}
\newcommand{\rappne}{\rulename{\apppref{}ne}}
\newcommand{\rappfun}{\rulename{\apppref{}fun}}
\newcommand{\rapppairl}{\rulename{\apppref{}pair-l}}
\newcommand{\rapppairr}{\rulename{\apppref{}pair-r}}

% type inference
\newcommand{\infpref}{inf-}
\newcommand{\rinfvar}{\rulename{\infpref{}var}}
\newcommand{\rinffune}{\rulename{\infpref{}fun-e}}
\newcommand{\rinfpairel}{\rulename{\infpref{}pair-e-l}}
\newcommand{\rinfpairer}{\rulename{\infpref{}pair-e-r}}

% type checking
\newcommand{\chkpref}{chk-}
\newcommand{\rchkinf}{\rulename{\chkpref{}inf}}
\newcommand{\rchkinff}{\rulename{\chkpref{}inf-f}}
%% \newcommand{\rchkcf}{\rulename{\chkpref{}{\sffamily c}-f}} %does
%% not work
\newcommand{\rchkcf}{\rulename{\chkpref{}c-f}}
\newcommand{\rchkdepf}{\rulename{\chkpref{}dep-f}}
\newcommand{\rchkfunf}{\rulename{\chkpref{}fun-f}}
\newcommand{\rchkfuni}{\rulename{\chkpref{}fun-i}}
\newcommand{\rchkpairf}{\rulename{\chkpref{}pair-f}}
\newcommand{\rchkpairi}{\rulename{\chkpref{}pair-i}}
\newcommand{\rchkset}{\rulename{\chkpref{}set}}
\newcommand{\rchksetf}{\rulename{\chkpref{}set-f}}
\newcommand{\rchksete}{\rulename{\chkpref{}set-e}}
%\newcommand{\rchk}{\rulename{\chkpref{}}}

% algorithmic equality
\newcommand{\aleqpref}{aq-}
\newcommand{\raleqbeta}{\rulename{\aleqpref{}\kern-0.2ex$\beta$}}
\newcommand{\raleqbetal}{\rulename{\aleqpref{}\kern-0.2ex$\beta$-l}}
\newcommand{\raleqbetar}{\rulename{\aleqpref{}\kern-0.2ex$\beta$-r}}
\newcommand{\raleqeta}{\rulename{\aleqpref{}$\eta$}}
\newcommand{\raleqext}{\rulename{\aleqpref{}ext}}
\newcommand{\raleqty}{\rulename{\aleqpref{}ty}}
\newcommand{\raleqtyne}{\rulename{\aleqpref{}ty-ne}}
\newcommand{\raleqtynat}{\rulename{\aleqpref{}ty-n}}
\newcommand{\raleqtyfun}{\rulename{\aleqpref{}ty-fun}}
\newcommand{\raleqtyset}{\rulename{\aleqpref{}ty-set}}
\newcommand{\raleqc}{\rulename{\aleqpref{}c}}
\newcommand{\raleqrec}{\rulename{\aleqpref{}rec}}
\newcommand{\raleqnate}{\rulename{\aleqpref{}n-e}}
\newcommand{\raleqnatiz}{\rulename{\aleqpref{}n-i-z}}
\newcommand{\raleqnatis}{\rulename{\aleqpref{}n-i-s}}
\newcommand{\raleqfix}{\rulename{\aleqpref{}fix}}
\newcommand{\raleqfixl}{\rulename{\aleqpref{}fix-l}}
\newcommand{\raleqfixr}{\rulename{\aleqpref{}fix-r}}
\newcommand{\raleqvar}{\rulename{\aleqpref{}var}}
\newcommand{\raleqatom}{\rulename{\aleqpref{}atom}}
\newcommand{\raleqne}{\rulename{\aleqpref{}ne}}
\newcommand{\raleqnef}{\rulename{\aleqpref{}ne-f}}
\newcommand{\raleqneatom}{\rulename{\aleqpref{}ne-atom}}
\newcommand{\raleqnefun}{\rulename{\aleqpref{}ne-fun}}
\newcommand{\raleqnepair}{\rulename{\aleqpref{}ne-pair}}
\newcommand{\raleqextfun}{\rulename{\aleqpref{}ext-fun}}
\newcommand{\raleqextfunfun}{\rulename{\aleqpref{}ext-fun-fun}}
\newcommand{\raleqextnefun}{\rulename{\aleqpref{}ext-ne-fun}}
\newcommand{\raleqextfunne}{\rulename{\aleqpref{}ext-fun-ne}}
\newcommand{\raleqextpair}{\rulename{\aleqpref{}ext-pair}}
\newcommand{\raleqextpairpair}{\rulename{\aleqpref{}ext-pair-pair}}
\newcommand{\raleqextnepair}{\rulename{\aleqpref{}ext-ne-pair}}
\newcommand{\raleqextpairne}{\rulename{\aleqpref{}ext-pair-ne}}
\newcommand{\raleqfunpair}{\rulename{\aleqpref{}fun-pair}}
\newcommand{\raleqpairfun}{\rulename{\aleqpref{}pair-fun}}
\newcommand{\raleqpi}{\rulename{\aleqpref{}$\Pi$}}
\newcommand{\raleqdep}{\rulename{\aleqpref{}dep}}
\newcommand{\raleqfun}{\rulename{\aleqpref{}fun}}
\newcommand{\raleqfune}{\rulename{\aleqpref{}fun}}
\newcommand{\raleqlam}{\rulename{\aleqpref{}$\lambda$}}
\newcommand{\raleqlaml}{\rulename{\aleqpref{}$\lambda$-l}}
\newcommand{\raleqlamr}{\rulename{\aleqpref{}$\lambda$-r}}
\newcommand{\raleqpair}{\rulename{\aleqpref{}pair}}
\newcommand{\raleqpairl}{\rulename{\aleqpref{}pair-l}}
\newcommand{\raleqpairr}{\rulename{\aleqpref{}pair-r}}
\newcommand{\raleqapp}{\rulename{\aleqpref{}\kern-0.2ex app}}
\newcommand{\raleqarr}{\rulename{\aleqpref{}$\to$}}
\newcommand{\raleqforall}{\rulename{\aleqpref{}\kern-0.3ex$\forall$}}
\newcommand{\raleqrefl}{\rulename{\aleqpref{}refl}}
\newcommand{\raleqsym}{\rulename{\aleqpref{}sym}}
\newcommand{\raleqtrans}{\rulename{\aleqpref{}trans}}

% reification
\newcommand{\rpref}{reify-}
\newcommand{\rrvar}{\rulename{\rpref{}var}}
\newcommand{\rrfune}{\rulename{\rpref{}fun-e}}
\newcommand{\rrnate}{\rulename{\rpref{}n-e}}
\newcommand{\rrne}{\rulename{\rpref{}ne}}
\newcommand{\rrext}{\rulename{\rpref{}ext}}
\newcommand{\rrnatiz}{\rulename{\rpref{}n-i-z}}
\newcommand{\rrnatis}{\rulename{\rpref{}n-i-s}}
\newcommand{\rrty}{\rulename{\rpref{}ty}}
\newcommand{\rrtyset}{\rulename{\rpref{}ty-set}}
\newcommand{\rrtynat}{\rulename{\rpref{}ty-n}}
\newcommand{\rrtyfun}{\rulename{\rpref{}ty-fun}}
\newcommand{\rrtyne}{\rulename{\rpref{}ty-ne}}
%\newcommand{\rr}{\rulename{\rpref{}}}


% inference and checking
\newcommand{\jne}{\Downarrow}
\newcommand{\jnf}{\Uparrow}
%\newcommand{\jinf}{\Downarrow}
%\newcommand{\jchk}{\Uparrow}
\newcommand{\jinf}{\rightrightarrows}
\newcommand{\jchk}{\leftleftarrows}
%\newcommand{\jinf}{\mathrel{\mathord{:}\mathord{\Rightarrow}}}
%\newcommand{\jchk}{\mathrel{\mathord{:}\mathord{\Leftarrow}}}
\newcommand{\ders}{\der_\mathsf{s}}

% normal and neutral
\newcommand{\neu}{\Downarrow}
\newcommand{\norm}{\Uparrow}

% model
\newcommand{\denpref}{den-}
\newcommand{\rdenvar}{\rulename{\denpref{}var}}
\newcommand{\rdenconst}{\rulename{\denpref{}const}}
\newcommand{\rdenconstr}{\rulename{\denpref{}constr}}
\newcommand{\rdenset}{\rulename{\denpref{}univ}}
\newcommand{\rdentype}{\rulename{\denpref{}type}}
\newcommand{\rdenel}{\rulename{\denpref{}el}}
\newcommand{\rdenfun}{\rulename{\denpref{}fun}}
\newcommand{\rdenpair}{\rulename{\denpref{}pair}}
%% these are deprecated:
%\newcommand{\rdeninvel}{\rulename{\denpref{}univ-f-inj}}
%\newcommand{\rdeninvfun}{\rulename{\denpref{}fun-f-inj}}
%\newcommand{\rdeninvpair}{\rulename{\denpref{}pair-f-inj}}
\newcommand{\rdenelinj}{\rulename{\denpref{}el-inj}}
\newcommand{\rdendepinj}{\rulename{\denpref{}dep-inj}}
\newcommand{\rdensetnotel}{\rulename{\denpref{}univ-not-el}}
\newcommand{\rdensetnotdep}{\rulename{\denpref{}univ-not-dep}}
\newcommand{\rdenelnotdep}{\rulename{\denpref{}el-not-dep}}
%\newcommand{\rdenseteinj}{\rulename{\denpref{}univ-e-inj}}
%\newcommand{\rdendepfinj}{\rulename{\denpref{}dep-f-inj}}
%\newcommand{\rdensetfnotsete}{\rulename{\denpref{}univ-f-not-set-e}}
%\newcommand{\rdensetfnotdep}{\rulename{\denpref{}set-f-not-dep-f}}
\newcommand{\rdenfune}{\rulename{\denpref{}fun-e}}
\newcommand{\rdenfuni}{\rulename{\denpref{}fun-i}}
\newcommand{\rdenalle}{\rulename{\denpref{}all-e}}
\newcommand{\rdenalli}{\rulename{\denpref{}all-i}}
\newcommand{\rdenpaire}{\rulename{\denpref{}pair-e}}
\newcommand{\rdenbeta}{\rulename{\denpref{}$\beta$}}
\newcommand{\rdenfunbeta}{\rulename{\denpref{}fun-$\beta$}}
\newcommand{\rdenpairbeta}{\rulename{\denpref{}pair-$\beta$}}
\newcommand{\rdenpairbetal}{\rulename{\denpref{}pair-$\beta$-l}}
\newcommand{\rdenpairbetar}{\rulename{\denpref{}pair-$\beta$-r}}
\newcommand{\rdenfunxi}{\rulename{\denpref{}fun-$\xi$}}
\newcommand{\rdenpairxi}{\rulename{\denpref{}pair-$\xi$}}
\newcommand{\rdenirr}{\rulename{\denpref{}irr}}
\newcommand{\rdensubst}{\rulename{\denpref{}subst}}
\newcommand{\rdentysubst}{\rulename{\denpref{}ty-subst}}
\newcommand{\rdeniotaz}{\rulename{\denpref{}$\iota$-z}}
\newcommand{\rdeniotas}{\rulename{\denpref{}$\iota$-s}}
\newcommand{\rdennate}{\rulename{\denpref{}\natpref{}e}}
%\newcommand{\rden}{\rulename{\denpref{}}}

% per model
\newcommand{\perpref}{per-}
\newcommand{\rper}[1]{\rulename{\perpref{}#1}}

% % projections
% \newcommand{\tL}{\mathsf{L}}
% \newcommand{\tR}{\mathsf{R}}

% % saturation interval
% \renewcommand{\N}{\mathcal{N}}
% \newcommand{\Sfun}{\mathcal{S}_{\mathit{fun}}}
% \newcommand{\Spair}{\mathcal{S}_{\mathit{pair}}}


% identitys
%\newcommand{\tid}{\mathsf{i\kern-0.1ex d}} % not such a good idea
\newcommand{\tid}{\mathsf{id}}
\newcommand{\tId}{\mathsf{Id}}
% identity substitution
%\newcommand{\sid}{\sigma_{\tid}}

% contexts
%\newcommand{\cempty}{\mathord{\triangledown}}
%\newcommand{\cempty}{\mathord{\diamond}}
%\newcommand{\cempty}{()}
\newcommand{\cempty}{\emptyset}
\newcommand{\cxt}{\ \mathsf{cxt}}

% calligraphic capital letters
\newcommand{\A}{\tycol{A}}
\newcommand{\B}{\tycol{B}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
%\newcommand{\G}{\mathcal{G}}
\renewcommand{\P}{\mathcal{P}}

% universes (semantically)
\newcommand{\UU}{\mathcal{U}}
\newcommand{\TT}{\TYPE}%{\mathcal{T}}

% models
%\newcommand{\R}{\mathcal{R}}
\newcommand{\Dom}{\mathsf{D}}
\newcommand{\Dne}{\mathsf{D}_{\mathsf{ne}}}
\newcommand{\Dnf}{\mathsf{D}_{\mathsf{nf}}}
\newcommand{\Deta}{\mathsf{D}^\eta}
\newcommand{\Rel}{\mathsf{Rel}}
\newcommand{\RelD}{\mathsf{Rel}(\Dom)}
\newcommand{\Per}{\mathsf{Per}}
\newcommand{\PerD}{\mathsf{Per}(\Dom)}
\newcommand{\Fam}{\mathsf{Fam}}
\newcommand{\EPer}{\mathfrak{EPer}}
\newcommand{\mapp}{\cdot}
\newcommand{\napp}{~}
\newcommand{\CXT}{\mathcal{C}\!\mathit{xt}}
\newcommand{\TYPE}{\mathcal{T}\!\mathit{ype}}
\newcommand{\SIZE}{\mathcal{S}\!\mathit{ize}}
\newcommand{\uTYPE}{\underline{\mathcal{T}\!\mathit{ype}}}
\newcommand{\EMPTY}{{\mathcal{E}\!\mathit{mpty}}}
\newcommand{\UNIT}{{\mathcal{U}\!\mathit{nit}}}
\newcommand{\NAT}{{\mathcal{N}\!\mathit{at}}}
\newcommand{\SET}[1][]{{\mathcal{S}\!\mathit{et}_{#1}}}
\newcommand{\el}[1]{[#1]}
\newcommand{\elt}[1]{#1}
\newcommand{\EL}[1][]{\mathcal{E}\kern-0.2ex\ell_{#1}}
\newcommand{\ELT}[1]{[#1]}
\newcommand{\ELC}[1]{[#1]}
\newcommand{\FUN}{\mathcal{F}\!\mathit{un}}
\newcommand{\PAIR}{\mathcal{P}\!\mathit{air}}
%\newcommand{\PI}[1]{\Pi\,#1\,}
\newcommand{\PI}{\prod}
\newcommand{\PIAF}{\PI\A\F}
\newcommand{\FORALL}{\forall}

\newcommand{\UP}{\mathop{\Uparrow}\nolimits^{\tkind}}
%\newcommand{\UP}{\mathop{\upuparrows}\nolimits}
\newcommand{\Up}[1]{\mathop{\Uparrow}\nolimits^{#1}}
%\newcommand{\up}[1]{\mathop{\uparrow}\nolimits^{#1}}
\newcommand{\up}[1]{\mathord{\uparrow^{#1}}}
%\newcommand{\upPi}[2]{\up{\piV{#1}{#2}}}

%\newcommand{\DOWN}{\mathop{\Downarrow}\nolimits^{\tkind}}
\newcommand{\DOWN}{\mathop{\downarrow}\nolimits}%\downdownarrows
\newcommand{\Down}[1]{\mathop{\Downarrow}\nolimits^{#1}}
\newcommand{\down}[1]{\mathord{\downarrow^{#1}}}
%\newcommand{\down}[1]{\mathop{\downarrow}\nolimits^{#1}}
\newcommand{\downPi}[2]{\down{\piV{#1}{#2}}}



% term model
\newcommand{\betaclass}[1]{\overline{#1}}
%\newcommand{\betaclass}[1]{\overline{#1}_{\beta}}
\newcommand{\betaeq}{=_\beta}
\newcommand{\etaeq}{=_\eta}
\newcommand{\biq}{=_{\beta\iota}}
\newcommand{\Expmod}{\Exp/\mathord{\betaeq}}



% algorithmic equality
%\newcommand{\cc}{^\mathsf{c}}
\newcommand{\wc}{_\mathsf{w}}

\newcommand{\tleft}{\mathsf{left}}
\newcommand{\tright}{\mathsf{right}}

% misc stuff
\newcommand{\sat}{\mathop{\mathsf{sat}}\nolimits}
\newcommand{\SN}{\mathsf{SN}}
\newcommand{\WN}{\mathsf{WN}}
\newcommand{\TmVar}{\mathsf{TmVar}}
\newcommand{\TyVar}{\mathsf{TyVar}}
\newcommand{\Subst}{\mathsf{Subst}}
\newcommand{\Eq}{\mathsf{Eq}} % for talkProgLog
\newcommand{\List}{\mathsf{List}}
\newcommand{\UList}{\mathsf{UList}}
\newcommand{\tappend}{\mathsf{append}}
\newcommand{\tvcons}{\mathsf{vcons}}
\newcommand{\tvnil}{\mathsf{vnil}}
\newcommand{\vxs}{\mathit{xs}}
\newcommand{\vys}{\mathit{ys}}
\newcommand{\vzs}{\mathit{zs}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% SemEq stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \renewcommand{\update}[3]{(#1,#2 \is #3)}
% \renewcommand{\subst}[3]{#3(\sid,#2 \is #1)}

% \renewcommand{\Den}[2]{#1 #2}
% \renewcommand{\den}[1]{#1\rid}

\newcommand{\comp}{\circ}

% de Bruijn index
\newcommand{\ind}[1]{\mathsf{v}_{#1}}
% de Bruijn level
\newcommand{\lev}[1]{\x_{#1}}
\newcommand{\var}[1]{\x_{#1}}
\newcommand{\xdel}[1][]{\ifthenelse{\equal{#1}{}}{\x_\Delta}{\x_{\Delta+#1}}}

% typing rules
\renewcommand{\ruf}{\rulename{\typref{}set-f}}
\renewcommand{\ruin}{\rulename{\typref{}set-i-n}}
\renewcommand{\ruifun}{\rulename{\typref{}set-i-fun}}
\renewcommand{\rue}{\rulename{\typref{}set-e}}
\newcommand{\rsub}{\rulename{\typref{}sub}} % subsumption

% typing rules for substitutions
\newcommand{\rsubstid}{\rulename{\substpref{}id}}
\newcommand{\rsubstcomp}{\rulename{\substpref{}comp}}
\newcommand{\rsubstweak}{\rulename{\substpref{}weak}}

% equality rules
\newcommand{\reqsub}{\rulename{\eqpref{}sub}} % subsumption


% equality rules for substitutions
\newcommand{\reqsubstidl}{\rulename{\eqsubstpref{}id-l}}
\newcommand{\reqsubstidr}{\rulename{\eqsubstpref{}id-r}}
\newcommand{\reqsubstassoc}{\rulename{\eqsubstpref{}assoc}}
\newcommand{\reqsubstemptybeta}{\rulename{\eqsubstpref{}empty-$\beta$}}
\newcommand{\reqsubstemptyeta}{\rulename{\eqsubstpref{}empty-$\eta$}}
\newcommand{\reqsubstextcomp}{\rulename{\eqsubstpref{}ext-comp}}
\newcommand{\reqsubstextbeta}{\rulename{\eqsubstpref{}ext-$\beta$}}
\newcommand{\reqsubstexteta}{\rulename{\eqsubstpref{}ext-$\eta$}}
\newcommand{\reqsubstextweak}{\rulename{\eqsubstpref{}ext-weak}}
\newcommand{\reqsubstid}{\rulename{\eqsubstpref{}id}}
\newcommand{\reqsubstcomp}{\rulename{\eqsubstpref{}comp}}
\newcommand{\reqsubstrefl}{\rulename{\eqsubstpref{}refl}}
\newcommand{\reqsubstsym}{\rulename{\eqsubstpref{}sym}}
\newcommand{\reqsubsttrans}{\rulename{\eqsubstpref{}trans}}
\newcommand{\reqsubstweak}{\rulename{\eqsubstpref{}weak}}
%\newcommand{\reqsubst}{\rulename{\eqsubstpref{}}}

% rules for handling of explicit substitutions
\newcommand{\esubstpref}{esubst-}
\newcommand{\resubstf}{\rulename{\esubstpref{}f}}

\newcommand{\eqesubstpref}{eq-esubst-}
\newcommand{\reqesubstf}{\rulename{\eqesubstpref{}f}}
\newcommand{\reqesubstconst}{\rulename{\eqesubstpref{}c}}
\newcommand{\reqesubstvar}{\rulename{\eqesubstpref{}var}}
\newcommand{\reqesubsthyp}{\rulename{\eqesubstpref{}var}}
\newcommand{\reqesubstweak}{\rulename{\eqesubstpref{}weak}}
\newcommand{\reqesubstfunf}{\rulename{\eqesubstpref{}fun-f}}
\newcommand{\reqesubstfuni}{\rulename{\eqesubstpref{}fun-i}}
\newcommand{\reqesubstfune}{\rulename{\eqesubstpref{}fun-e}}
\newcommand{\reqesubstid}{\rulename{\eqesubstpref{}id}}
\newcommand{\reqesubstcomp}{\rulename{\eqesubstpref{}comp}}
%\newcommand{\reqesubst}{\rulename{\eqesubstpref{}}}



\newcommand{\D}{\mathcal{D}}

% evaluation and application laws (already in macros)
%\newcommand{\evalpref}{eval-}
\newcommand{\revalconst}{\rulename{\evalpref{}c}}
%\newcommand{\revalvar}{\rulename{\evalpref{}var}}
%\newcommand{\revalfune}{\rulename{\evalpref{}fun-e}}
\newcommand{\revalesubst}{\rulename{\evalpref{}esubst}}
%\newcommand{\reval}{\rulename{\evalpref{}}}

\newcommand{\evalsubstpref}{eval-subst-}
\newcommand{\revalsubstid}{\rulename{\evalsubstpref{}id}}
\newcommand{\revalsubstcomp}{\rulename{\evalsubstpref{}comp}}
\newcommand{\revalsubstempty}{\rulename{\evalsubstpref{}empty}}
\newcommand{\revalsubstext}{\rulename{\evalsubstpref{}ext}}
%\newcommand{\revalsubst}{\rulename{\evalsubstpref{}}}

\renewcommand{\apppref}{app-}
\newcommand{\rappfuni}{\rulename{\apppref{}fun-i}}
\renewcommand{\rappne}{\rulename{\apppref{}ne}}
%\newcommand{\rapp}{\rulename{\app{}}}
\newcommand{\rapprecz}{\rulename{\apppref{}rec-z}}
\newcommand{\rapprecs}{\rulename{\apppref{}rec-s}}

% reevaluation and application laws (already in macros)
\newcommand{\reevalpref}{reeval-}
\newcommand{\rreevalconst}{\rulename{\reevalpref{}c}}
\newcommand{\rreevalvar}{\rulename{\reevalpref{}var}}
\newcommand{\rreevalfune}{\rulename{\reevalpref{}fun-e}}
\newcommand{\rreevalesubst}{\rulename{\reevalpref{}esubst}}
\newcommand{\rreevalid}{\rulename{\reevalpref{}id}}
%\newcommand{\rreeval}{\rulename{\reevalpref{}}}

% renaming
\newcommand{\renpref}{ren-}
\newcommand{\rrenconst}{\rulename{\renpref{}c}}
\newcommand{\rrenvar}{\rulename{\renpref{}var}}
\newcommand{\rrenapp}{\rulename{\renpref{}app}}
\newcommand{\rreneval}{\rulename{\renpref{}eval}}
\newcommand{\rrenne}{\rulename{\renpref{}ne}}
\newcommand{\rrenneapp}{\rulename{\renpref{}neapp}}
\newcommand{\rrennerec}{\rulename{\renpref{}nerec}}
\newcommand{\rrencxtempty}{\rulename{\renpref{}cxt-empty}}
\newcommand{\rrencxtext}{\rulename{\renpref{}cxt-ext}}
%\newcommand{\rren}{\rulename{\renpref{}}}

%cumulativity relation
\newcommand{\cum}{\preccurlyeq}
\newcommand{\cocum}{\succcurlyeq}

% Kripke model
%\renewcommand{\circledS}{\ensuremath{\mathrel{\textcircled{\scriptsize=}}}}
%\renewcommand{\circledS}{\ensuremath{\mathrel{\textcircled{e}}}}
%\renewcommand{\circledS}{\ensuremath{\mathrel{\fbox{K}}}}
\newcommand{\Seq}{\mathrel{\circledS}}
\newcommand{\Ceq}{\mathrel{\copyright}}
\newcommand{\circlerel}[1]{%
  \mathrel{\ensuremath{\textcircled{\ensuremath{#1}}}}%
}
\newcommand{\Seqcum}{\circlerel{\cum}}
\newcommand{\Seqcocum}{\circlerel{\cocum}}

\newcommand{\closerel}[1]{\mathrel{\close{\small#1}}}
\newcommand{\cleq}{\closerel{\Seq}}
\newcommand{\cleqcum}{\closerel{\Seqcum}}
\newcommand{\cleqcocum}{\closerel{\Seqcocum}}

%the raisebox is ignored, why?
\newcommand{\Cleq}{\mathrel{\ensuremath{\raisebox{2pt}{\ensuremath{\close{\raisebox{-2pt}{\ensuremath{\Ceq}}}}}}}}
\newcommand{\Ceqcum}{\stackrel{c}{\Seqcum}}
\newcommand{\Cleqcum}{\stackrel{\close{c}}{\Seqcum}}
\newcommand{\Ceqcocum}{\stackrel{c}{\Seqcocum}}
\newcommand{\Cleqcocum}{\stackrel{\close{c}}{\Seqcocum}}


\newcommand{\circleEq}{\mathrel{\circledS}}%\circeq
\newcommand{\EQ}[6]{#1 \der #2 : #3 \circleEq  #4 \der #5 : #6}
\newcommand{\EQE}[5]{#1 \der #2 \circleEq  #4 \der #5 :: #3}
\newcommand{\EQC}[5]{#1 \der #2 \circleEq  #3 \der #4 :: #5}
% \newcommand{\EQE}[5]{#1 \der #2 : #3 \circleEq  #4 \der #5}
% \newcommand{\EQC}[5]{#1 \der #2 : #5 \circleEq  #3 \der #4}
\newcommand{\KRel}{\mathsf{KRel}}
\newcommand{\SemCxt}{\mathsf{SemCxt}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\NEE}{\mathcal{N}\!\mathcal{E}}
\newcommand{\NE}{\mathcal{N}\!\mathit{e}}
\newcommand{\NF}{\mathcal{N}\!\mathit{f}}
\newcommand{\ELIM}{\mathcal{E}\!\mathit{lim}}
\newcommand{\TY}{\mathcal{T}\!\mathit{y}}
\newcommand{\Index}{\mathsf{Index}}

\newcommand{\RO}{\mathcal{R}}
\newcommand{\RR}{\mathrel{\RO}}

%\newcommand{\Bool}{\mathsf{Bool}}
\newcommand{\ttrue}{\mathsf{true}}
\newcommand{\tfalse}{\mathsf{false}}


% % logical relation
% \newcommand{\circleR}{\mathrel{\mbox{\textregistered}}}
% \newcommand{\LR}[5]{#1 \der #2 : #3 \circleR #4 \in #5}
% \newcommand{\LRS}[4]{#1 \der #2 : #3 \circleR #4}
% \newcommand{\LRSub}[6]{#1 \der #2 \eeq #3 : #4 \circleR #5 \eeq #6}
% \newcommand{\LRSize}[3]{#1 \der #2 \doteq \tRsize #3}
% %\newcommand{\LRSize}[3]{#1 \der #2 : \Size \circleR #3}
% \newcommand{\LRTS}[4]{#1 \der #2 \circleR #3 \in #4}
% \newcommand{\LRT}[4]{#1 \der #2 \circleR #3 \in \Set[#4]}
% %\newcommand{\RG}[5]{#1 \der #2 \circleR #4 \der #5 :: #3}
% \newcommand{\RG}[3]{#1 \der #2  \circleR #3}
% \newcommand{\TyG}[1]{\Ty(#1)}
% \newcommand{\TmG}[2]{\Tm(#1,#2)}

\newcommand{\RNE}[4]{#1 \der #2 \doteq \tRne\, #3 : #4}
\newcommand{\RD}[4]{#1 \der #2 \doteq \tR\, #3 : #4}
\newcommand{\RTY}[4]{#1 \der #2 \doteq \tRty\, #3 : #4}
\newcommand{\RSIZE}[3]{#1 \der #2 \doteq \tRsize #3}


%\newcommand{\VDash}{\mathrel{\mathord{|}\kern-0.15ex\mathord{\models}}}
%\newcommand{\VvDash}{\mathrel{||\mathord{\vDash}}}

\newcommand{\valic}{\Vdash^\mathsf{c}}
\newcommand{\valid}{\Vdash}
\newcommand{\svalid}{\VDash}
\renewcommand{\sat}{\Vvdash}

% semantical typing
\newcommand{\dersem}{\models}
\newcommand{\jsem}{:}
\newcommand{\seq}[4]{#1 \dersem #2 = #3 \jsem #4}
\newcommand{\swf}[3]{#1 \dersem #2 \jsem #3}
\newcommand{\steq}[3]{#1 \dersem #2 = #3}
\newcommand{\stwf}[2]{#1 \dersem #2}
\newcommand{\sceq}[2]{\dersem #1 = #2}
\newcommand{\scwf}[1]{\dersem #1}

% logical relation
\newcommand{\steqd}[5]{#1 \valid #2 = #3 : \SET[#4] /_{#5}}
\newcommand{\sttmd}[4]{#1 \valid #2 : #3 /_{#4}}
\newcommand{\stmeqd}[5]{#1 \valid #2 = #3 : #4 /_{#5}}
\newcommand{\sttmeqd}[6]{#1 \valid #2 = #3 : #4 /_{#5}}
\newcommand{\snat}[3]{#1 \valid #2 : \NAT(#3)}
\newcommand{\snateq}[4]{#1 \valid #2 = #3 : \NAT(#4)}
\newcommand{\sneq}[4]{#1 \valid #2 = #3 : \NE(#4)}
\newcommand{\cevalsto}{\mathrel{{}_{:}\!\!\!\evalsto\!\!\!^{:}}}

% lambda model
\newcommand{\eid}{\eta_{\tid}}
\newcommand{\rid}{\rho_{\tid}}
\newcommand{\clam}[3]{(\lambda #1#2)#3}

% reification
\newcommand{\reifiesto}{\searrow}
%\newcommand{\Nbe}[1][]{\mathop{\mathsf{Nbe}}\nolimits_{#1}}
%\newcommand{\R}[1][]{\mathop{\mathsf{R}_{#1}}\nolimits}
%\newcommand{\Read}[1]{\R{#1}^\ttype}
%\newcommand{\READ}[1]{\R{#1}^\box}
\newcommand{\rchk}[4]{#1 \der #2 \searrow #3 \jchk #4}
\newcommand{\rinf}[4]{#1 \der #2 \searrow #3 \jinf #4}
\newcommand{\rr}[4]{#1 \der #2 \searrow #3 \RR #4}
\newcommand{\rcxt}[2]{#1 \searrow #2}
% \SUBTYPING{
% \newcommand{\rty}[4]{#1 \der #2 \searrow #3 \jchk \SetD \leadsto #4}
% }\NOSUBTYPING{
% \newcommand{\rty}[4]{#1 \der #2 \searrow #3 \jchk \SetD_{#4}}
% }
% % equality algorithm
% \SUBTYPING{
% \newcommand{\eqty}[4]{#1 \der #2 = #3 \jchk \SetD \leadsto #4}
% }\NOSUBTYPING{
% \newcommand{\eqty}[4]{#1 \der #2 = #3 \jchk \SetD_{#4}}
% }

% type checking algorithm
% \SUBTYPING{
% \newcommand{\chkty}[4]{#1 \der #2\ #3 \jchk \SetD \leadsto #4}
% }\NOSUBTYPING{
% \newcommand{\chkty}[4]{#1 \der #2\ #3 \jchk \SetD_{#4}}
% }
\newcommand{\did}{\delta_{\tid}}



\newcommand{\N}[1][]{\mathsf{N}_{#1}}
\newcommand{\W}{\mathcal{W}}












% tables and figures
% deftable, deffigure, figureone, figuretwo, figuretwosqueeze

%Tables
\newenvironment{deftable}[2]{%
  \def\deftablecaption{#2}%
  \begin{table}[htbp]%
  \begin{center}%
  \begin{scriptsize}%
  \begin{minipage}{#1}%
  \hrule \vspace*{4ex}%
%  % reassign dimensions for prooftrees
%  \proofrulebaseline=2ex%
%  \proofrulebreadth=.05em%
%  \proofdotseparation=1.25ex%
}{%
\vspace{2ex} \hrule%
\addvspace{2ex}%
  \end{minipage}%
  \end{scriptsize}%
  \end{center}%
  \caption{\deftablecaption}%
  \end{table}%
}

%Figures
\newenvironment{deffigure}[2]{%
  \def\deffigurecaption{#2}%
  \begin{figure*}[htbp]%
  \begin{center}%
  %\begin{scriptsize}%
  \begin{minipage}{#1}%
  \hrule \vspace*{4ex}%
%  % reassign dimensions for prooftrees
%  \proofrulebaseline=2ex%
%  \proofrulebreadth=.05em%
%  \proofdotseparation=1.25ex%
}{%
\vspace{2ex} \hrule%
\addvspace{2ex}%
  \end{minipage}%
  %\end{scriptsize}%
  \end{center}%
  \caption{\deffigurecaption}%
  \end{figure*}%
}

\newenvironment{figureone}[1]{%
  \def\deffigurecaption{#1}%
  \begin{figure}[htbp]%
  \begin{center}%
  %\begin{scriptsize}%
  \begin{minipage}{\columnwidth}%
  \hrule \vspace*{2ex}%
  % reassign dimensions for prooftrees
  \proofrulebaseline=2ex%
  \proofrulebreadth=.05em%
  \proofdotseparation=1.25ex%
}{%
\vspace{2ex} \hrule%
%\addvspace{2ex}%
  \end{minipage}%
  %\end{scriptsize}%
  \end{center}%
  \caption{\deffigurecaption}%
  \end{figure}%
}

\newenvironment{figuretwo}[1]{%
  \def\deffigurecaption{#1}%
  \begin{figure*}[htbp]%
  \begin{center}%
  %\begin{scriptsize}%
  \begin{minipage}{\textwidth}%
  \hrule \vspace*{2ex}%
  % reassign dimensions for prooftrees
  \proofrulebaseline=2ex%
  \proofrulebreadth=.05em%
  \proofdotseparation=1.25ex%
}{%
%\vspace{2ex}
  \hrule%
%\addvspace{2ex}%
  \end{minipage}%
  %\end{scriptsize}%
  \end{center}%
  \caption{\deffigurecaption}%
  \end{figure*}%
}

\newenvironment{figuretwosqueeze}[1]{%
  \def\deffigurecaption{#1}%
  \begin{figure*}[htbp]%
  \begin{center}%
  %\begin{scriptsize}%
  \begin{minipage}{\textwidth}%
  \hrule \vspace*{2ex}%
  % reassign dimensions for prooftrees
  \proofrulebaseline=2ex%
  \proofrulebreadth=.05em%
  \proofdotseparation=1.25ex%
}{%
%\vspace{2ex}
\hrule%
%\addvspace{2ex}%
  \end{minipage}%
  %\end{scriptsize}%
  \end{center}%
  \caption{\deffigurecaption}%
  \end{figure*}%
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "icfp18"
%%% End:


==> moldy/closing_main.tex <==

\immediate\closeout\boxesfile

==> moldy/combination_term.tex <==
\tlet{\TBOX{\bar{p}}{\mathit{x}}}{\mathit{handler}}{\TUNBOX{p}\app{(\lam{()}{\mathit{program}})}\app{\TBOX{\bar{p}}{\mathit{x}}}}

==> moldy/combination_type.tex <==
\mathit{A}⊸\mathit{B}\text{, ~if~}\mathit{ε} : \mathit{q}\mathit{p}\convertible{}1\text{, ~if~}\mathit{η} : 1\convertible{}\mathit{p}\mathit{q}

==> moldy/conv_term.tex <==
\lam{\TBOX{\mathnormal{p}}{\pconv{\mathnormal{ϕ}}{\mathnormal{x}}}}{\TBOX{\mathnormal{q}}{\mathnormal{x}}}

==> moldy/dupUnit_term.tex <==
\lam{()}{((),())}

==> moldy/dupUnit_type.tex <==
1⊸1⊗1

==> moldy/fourtytwo_type.tex <==
\mathit{ℕ}

==> moldy/get_type.tex <==
\BOX{\mathit{p}}\mathit{ℕ}

==> moldy/graded_bind_term.tex <==
\lam{\TBOX{\mathit{p}}{\mathit{x}}}{\lam{\TBOX{\mathit{p}}{\mathit{f}}}{\tlet{\TBOX{\mathit{p}}{\TBOX{\mathit{q}}{\mathit{y}}}}{\TBOX{\mathit{p}}{\mathit{f}\app{\mathit{x}}}}{\TBOX{\mathit{p}\mathit{q}}{\mathit{y}}}}}

==> moldy/graded_bind_type.tex <==
\BOX{\mathit{p}}\mathit{A}⊸\BOX{\mathit{p}}(\mathit{A}⊸\BOX{\mathit{q}}\mathit{B})⊸\BOX{\mathit{p}\mathit{q}}\mathit{B}

==> moldy/handler_type.tex <==
\mathit{A}⊸\BOX{\mathit{p}}1

==> moldy/inc_type.tex <==
\mathit{ℕ}⊸\mathit{ℕ}

==> moldy/mul_type.tex <==
\mathit{ℕ}⊸\mathit{ℕ}⊸\mathit{ℕ}

==> moldy/newunicodedefs.tex <==
% \newunicodechar{↝}{\ensuremath{\leadsto}}
%\newunicodechar{⁺}{^+}
%\newunicodechar{₁}{_1}
%\newunicodechar{₂}{_2}
\DeclareMathAlphabet{\mymathds}{U}{BOONDOX-ds}{m}{n}
\newcommand\llbrace{\mathopen{{\{\kern-0.24em|}}}    % opening {{ value delimiter
\newcommand\rrbrace{\mathclose{{|\kern-0.24em\}}}}   % closing }} value delimiter
\newcommand{\bidirmultimap}{\mathrel{\ooalign{$\mkern6mu\multimap$\cr$\reflectbox{\(\multimap\)}$\cr}}}
\newunicodechar{ }{{\,}}
\newunicodechar{¬}{\ensuremath{\neg}} %
\newunicodechar{²}{^2}
\newunicodechar{³}{^3}
\newunicodechar{·}{\ensuremath{\cdot}}
\newunicodechar{¹}{^1}
\newunicodechar{×}{\ensuremath{\times}} %
\newunicodechar{÷}{\ensuremath{\div}} %
\newunicodechar{ʳ}{^r}
\newunicodechar{ˡ}{^l}
\newunicodechar{Γ}{\Gamma}   %
\newunicodechar{Δ}{\ensuremath{\Delta}} %
\newunicodechar{Η}{\ensuremath{\textrm{H}}} %
\newunicodechar{Θ}{\ensuremath{\Theta}} %
\newunicodechar{Λ}{\ensuremath{\Lambda}} %
\newunicodechar{Ξ}{\ensuremath{\Xi}} %
\newunicodechar{Π}{\ensuremath{\Pi}}   %
\newunicodechar{Σ}{\ensuremath{\Sigma}} %
\newunicodechar{Φ}{\ensuremath{\Phi}} %
\newunicodechar{Ψ}{\ensuremath{\Psi}} %
\newunicodechar{Ω}{\ensuremath{\Omega}} %
\newunicodechar{α}{\ensuremath{\mathnormal{\alpha}}} %
\newunicodechar{β}{\ensuremath{\beta}} %
\newunicodechar{γ}{\ensuremath{\mathnormal{\gamma}}} %
\newunicodechar{δ}{\ensuremath{\mathnormal{\delta}}} %
\newunicodechar{ε}{\ensuremath{\mathnormal{\varepsilon}}} %
\newunicodechar{ζ}{\ensuremath{\mathnormal{\zeta}}} %
\newunicodechar{η}{\ensuremath{\mathnormal{\eta}}} %
\newunicodechar{θ}{\ensuremath{\mathnormal{\theta}}} %
\newunicodechar{ι}{\ensuremath{\mathnormal{\iota}}} %
\newunicodechar{κ}{\ensuremath{\mathnormal{\kappa}}} %
\newunicodechar{λ}{\ensuremath{\mathnormal{\lambda}}} %
\newunicodechar{μ}{\ensuremath{\mathnormal{\mu}}} %
\newunicodechar{ν}{\ensuremath{\mathnormal{\mu}}} %
\newunicodechar{ξ}{\ensuremath{\mathnormal{\xi}}} %
\newunicodechar{π}{\ensuremath{\mathnormal{\pi}}} %
\newunicodechar{ρ}{\ensuremath{\mathnormal{\rho}}} %
\newunicodechar{σ}{\ensuremath{\mathnormal{\sigma}}} %
\newunicodechar{τ}{\ensuremath{\mathnormal{\tau}}} %
\newunicodechar{φ}{\ensuremath{\mathnormal{\varphi}}} %
\newunicodechar{χ}{\ensuremath{\mathnormal{\chi}}} %
\newunicodechar{ψ}{\ensuremath{\mathnormal{\psi}}} %
\newunicodechar{ω}{\ensuremath{\mathnormal{\omega}}} %
\newunicodechar{ϕ}{\ensuremath{\mathnormal{\phi}}} %
\newunicodechar{ϵ}{\ensuremath{\mathnormal{\epsilon}}} %
\newunicodechar{ᵏ}{^k}
\newunicodechar{ᵢ}{_i} %
\newunicodechar{•}{\ensuremath{\cdot}} %
\newunicodechar{ }{{\,}}
\newunicodechar{′}{\ensuremath{^\prime}}  %
\newunicodechar{″}{\ensuremath{^\second}} %
\newunicodechar{‴}{\ensuremath{^\third}}  %
\newunicodechar{ⁱ}{^i}
\newunicodechar{⁵}{\ensuremath{^5}}
\newunicodechar{⁺}{\ensuremath{^+}} %%
\newunicodechar{⁻}{\ensuremath{^-}} %%
\newunicodechar{ⁿ}{^n}
\newunicodechar{₀}{\ensuremath{_0}} %
\newunicodechar{₁}{\ensuremath{_1}}
\newunicodechar{₂}{\ensuremath{_2}}
\newunicodechar{₃}{_3}
\newunicodechar{₊}{\ensuremath{_+}} %%
\newunicodechar{₋}{\ensuremath{_-}} %%
\newunicodechar{ₙ}{_n}
\newunicodechar{ₚ}{_p} %
\newunicodechar{ℂ}{\ensuremath{\mathds{C}}} %
\newunicodechar{ℕ}{\mathbb{N}} %
\newunicodechar{ℝ}{\ensuremath{\mathbb{R}}} %
\newunicodechar{ℤ}{\ensuremath{\mathbb{Z}}} %
\newunicodechar{ℳ}{\mathcal{M}}
\newunicodechar{⅋}{\ensuremath{\parr}} %
\newunicodechar{←}{\ensuremath{\leftarrow}} %
\newunicodechar{↑}{\ensuremath{\uparrow}} %
\newunicodechar{↓}{\ensuremath{\downarrow}} %
\newunicodechar{→}{\ensuremath{\rightarrow}} %
\newunicodechar{↔}{\ensuremath{\leftrightarrow}} %
\newunicodechar{↖}{\nwarrow} %
\newunicodechar{↗}{\nearrow} %
\newunicodechar{↝}{\ensuremath{\rightsquigarrow}}
\newunicodechar{↦}{\ensuremath{\mapsto}}
\newunicodechar{↭}{\ensuremath{\leftrightsquigarrow}} %
\newunicodechar{↾}{\ensuremath{\upharpoonright}} %
\newunicodechar{⇆}{\ensuremath{\leftrightarrows}} %
\newunicodechar{⇐}{\ensuremath{\Leftarrow}} %
\newunicodechar{⇒}{\ensuremath{\Rightarrow}} %
\newunicodechar{⇔}{\ensuremath{\Leftrightarrow}} %
\newunicodechar{∀}{\ensuremath{\forall}}   %
\newunicodechar{∃}{\ensuremath{\exists}} %
\newunicodechar{∅}{\ensuremath{\varnothing}} %
\newunicodechar{∈}{\ensuremath{\in}}
\newunicodechar{∉}{\ensuremath{\not\in}} %
\newunicodechar{∋}{\ensuremath{\ni}}  %
\newunicodechar{∎}{\ensuremath{\qed}}
\newunicodechar{∏}{\prod}
\newunicodechar{∑}{\sum}
\newunicodechar{∗}{\ensuremath{\ast}} %
\newunicodechar{∘}{\ensuremath{\circ}} %
\newunicodechar{∙}{\ensuremath{\bullet}} %
\newunicodechar{∙}{\ensuremath{\cdot}}
\newunicodechar{∞}{\ensuremath{\infty}} %
\newunicodechar{∣}{\ensuremath{\mid}} %
\newunicodechar{∧}{\ensuremath{\wedge}}%
\newunicodechar{∨}{\ensuremath{\vee}}%
\newunicodechar{∩}{\ensuremath{\cap}} %
\newunicodechar{∪}{\ensuremath{\cup}} %
\newunicodechar{∫}{\int}
\newunicodechar{∷}{::} %
\newunicodechar{∼}{\ensuremath{\sim}} %
\newunicodechar{≃}{\ensuremath{\simeq}} %
\newunicodechar{≅}{\ensuremath{\cong}} %
\newunicodechar{≈}{\ensuremath{\approx}} %
\newunicodechar{≔}{:=} %
\newunicodechar{≜}{\ensuremath{\stackrel{\scriptscriptstyle {\triangle}}{=}}}
\newunicodechar{≜}{\triangleq}
\newunicodechar{≝}{\ensuremath{\stackrel{\scriptscriptstyle {\text{def}}}{=}}}
\newunicodechar{≟}{\ensuremath{\stackrel {_\text{\textbf{?}}}{\text{\textbf{=}}\negthickspace\negthickspace\text{\textbf{=}}}}}
\newunicodechar{≠}{\ensuremath{\neq}}%
\newunicodechar{≡}{\ensuremath{\equiv}}%
\newunicodechar{≤}{\ensuremath{\leq}} %
\newunicodechar{≥}{\ensuremath{\geq}} %
\newunicodechar{≺}{\ensuremath{\prec}}
\newunicodechar{≼}{\ensuremath{\preceq}}
\newunicodechar{⊂}{\ensuremath{\subset}} %
\newunicodechar{⊃}{\ensuremath{\supset}} %
\newunicodechar{⊆}{\ensuremath{\subseteq}} %
\newunicodechar{⊇}{\ensuremath{\supseteq}} %
\newunicodechar{⊎}{\ensuremath{\uplus}} %
\newunicodechar{⊑}{\ensuremath{\sqsubseteq}} %
\newunicodechar{⊒}{\ensuremath{\sqsupseteq}} %
\newunicodechar{⊓}{\ensuremath{\sqcap}} %
\newunicodechar{⊔}{\ensuremath{\sqcup}} %
\newunicodechar{⊕}{\ensuremath{\oplus}} %
\newunicodechar{⊗}{\ensuremath{\otimes}} %
\newunicodechar{⊞}{\ensuremath{\boxplus}} %
\newunicodechar{⊟}{\ensuremath{\boxminus}} %
\newunicodechar{⊡}{\ensuremath{\boxdot}} %
\newunicodechar{⊢}{\ensuremath{\vdash}} %
\newunicodechar{⊣}{\ensuremath{\dashv}}
\newunicodechar{⊤}{\ensuremath{\top}}%
\newunicodechar{⊥}{\ensuremath{\bot}} % bottom
\newunicodechar{⊧}{\vDash} %
\newunicodechar{⊨}{\vDash} %
\newunicodechar{⊩}{\Vdash}
\newunicodechar{⊸}{\ensuremath{\multimap}} %
\newunicodechar{⋁}{\ensuremath{\bigvee}}
\newunicodechar{⋃}{\ensuremath{\bigcup}} %
\newunicodechar{⋄}{\ensuremath{\diamond}} %
\newunicodechar{⋆}{\ensuremath{\star}} %
\newunicodechar{⋮}{\ensuremath{\vdots}} %
\newunicodechar{⋯}{\ensuremath{\cdots}} %
\newunicodechar{─}{---}
\newunicodechar{□}{\ensuremath{\Box}} %
\newunicodechar{▹}{\ensuremath{\rhd}} %
\newunicodechar{◂}{\ensuremath{\triangleleft}}
\newunicodechar{◃}{\triangleleft{}} %
\newunicodechar{◆}{\blacklozenge} %
\newunicodechar{◇}{\ensuremath{\Diamond}} %
\newunicodechar{◽}{\ensuremath{\square}} %
\newunicodechar{★}{\ensuremath{\star}}   %
\newunicodechar{♢}{\ensuremath{\diamondsuit}} %
\newunicodechar{♭}{\ensuremath{\flat}} %
\newunicodechar{♯}{\ensuremath{\sharp}} %
\newunicodechar{✓}{\ensuremath{\checkmark}} %
\newunicodechar{⟂}{\ensuremath{\bot}} % PERPENDICULAR
\newunicodechar{⟦}{\ensuremath{\llbracket}}
\newunicodechar{⟧}{\ensuremath{\rrbracket}}
\newunicodechar{⟨}{\ensuremath{\langle}} %
\newunicodechar{⟩}{\ensuremath{\rangle}} %
\newunicodechar{⟶}{\ensuremath{\longrightarrow}}
\newunicodechar{⟷}{\longleftrightarrow}
\newunicodechar{⟹}{\ensuremath{\Longrightarrow}} %
\newunicodechar{⦃}{\ensuremath{\llbrace}} %
\newunicodechar{⦄}{\ensuremath{\rrbrace}} %
\newunicodechar{⧟}{\ensuremath{\bidirmultimap}} %
\newunicodechar{⨁}{\bigoplus} %
\newunicodechar{⨂}{\bigotimes} %
\newunicodechar{⫪}{\ensuremath{\top\kern-1.3ex\top}}
\newunicodechar{ⱼ}{_j} %
\newunicodechar{𝒟}{\ensuremath{\mathcal{D}}} %
\newunicodechar{𝒢}{\ensuremath{\mathcal{G}}}
\newunicodechar{𝒦}{\ensuremath{\mathcal{K}}} %
\newunicodechar{𝔸}{\ensuremath{\mathds{A}}} %
\newunicodechar{𝔹}{\ensuremath{\mathds{B}}} %
\newunicodechar{𝟘}{\ensuremath{\mymathds{0}}} %
\newunicodechar{𝟙}{\ensuremath{\mymathds{1}}} %


==> moldy/normie_red_term.tex <==
\lam{\TBOX{\mathit{p}}{(\mathit{x},\mathit{f})}}{\TBOX{\mathit{p}}{\mathit{f}\app{\mathit{x}}}}

==> moldy/normie_red_type.tex <==
\BOX{\mathit{p}}(\mathit{A}⊗(\mathit{A}⊸\mathit{B}))⊸\BOX{\mathit{p}}\mathit{B}

==> moldy/normie_term.tex <==
\mathit{functor_principle}\app{(\lam{(\mathit{x},\mathit{f})}{\mathit{f}\app{\mathit{x}}})}

==> moldy/normie_type.tex <==
\BOX{\mathit{p}}(\mathit{A}⊗(\mathit{A}⊸\mathit{B}))⊸\BOX{\mathit{p}}\mathit{B}

==> moldy/plus_type.tex <==
\mathit{ℕ}⊸\mathit{ℕ}⊸\mathit{ℕ}

==> moldy/pointWiseSum_term.tex <==
\lam{\TBOX{\mathit{p}}{\mathit{x}}}{\lam{\TBOX{\mathit{p}}{\mathit{y}}}{\TBOX{\mathit{p}}{\mathit{plus}\app{\mathit{x}}\app{\mathit{y}}}}}

==> moldy/pointWiseSum_type.tex <==
\BOX{\mathit{p}}\mathit{ℕ}⊸\BOX{\mathit{p}}\mathit{ℕ}⊸\BOX{\mathit{p}}\mathit{ℕ}

==> moldy/program_type.tex <==
\BOX{\mathit{p}}\mathit{A}

==> moldy/put_type.tex <==
\mathit{ℕ}⊸\BOX{\mathit{p}}1

==> moldy/replicate_type.tex <==
\mathit{ℕ}⊸\BOX{\mathit{p}}\mathit{ℕ}

==> moldy/sum_term.tex <==
\lam{\TBOX{\mathit{p}}{\mathit{x}}}{\lam{\TBOX{\mathit{p}}{\mathit{y}}}{\TBOX{\mathit{p}}{\mathit{plus}\app{\mathit{x}}\app{\mathit{y}}}}}

==> syntaxMacros.tex <==
%% \RequirePackage{mathabx} % \otop  %% UGLY
\RequirePackage{stmaryrd}
\RequirePackage{xspace}
\RequirePackage{tikz}  %% FOR circled

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
   \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\providecommand\basetype{\mathit{b}} % WAS: mathsf
\newcommand{\TyConst}{\beta}
\newcommand{\TyVar}{\mathsf{TyVar}}
\newcommand{\Ty}{\mathsf{Ty}}
\newcommand{\Tm}{\mathsf{Tm}}
\newcommand{\Cxt}{\mathsf{Cxt}}
\newcommand{\ModVar}{\mathsf{ModVar}}
\newcommand{\ModExp}{\mathsf{ModExp}}
% \newcommand{\land}{\wedge}

\newcommand\mbraces[1]{⦃ #1 ⦄}
\newcommand\braces[1]{\{ #1 \}}
\newcommand\setcomp[2]{\braces{ #1 ∣ #2 }}
\newcommand\VAR{}

\newcommand\funOpBidir{⧟}
% \newcommand\fun[2][]{\moda{#1}#2 \to}
% \newcommand\app[1][]{\moda{#1}}
% \newcommand\lam[2][]{\lambda\moda{#1} #2.}


\newcommand\use[2]{#1#2}
\newcommand\entail[4]{#1#2 ⊢ #3 : #4}

\newcommand{\bla}{\ensuremath{\mbox{$$}}} % invisible, but not ignored

\newcommand{\tReal}{\mathsf{Real}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Rinf}{\Real^{\infty}_{\geq 0}}
\newcommand{\Rpos}{\Real_{\geq 0}}
\newcommand{\Pol}{\mathsf{Pol}}
\newcommand{\dotsquare}{\boxdot}

\newcommand{\Bool}{\mathsf{Bool}}
\newcommand{\ttrue}{\mathsf{true}}
\newcommand{\tfalse}{\mathsf{false}}
\newcommand{\tcase}{\mathsf{case}}
\newcommand{\dup}{\mathsf{dup}}

\newcommand{\ClMonoTy}{\mathsf{Ty_0^0}}
\newcommand{\MonoTy}{\mathsf{Ty_0}}
\newcommand{\Mod}{\mathsf{Mod}}
\newcommand{\update}[3]{#1[#2 \mapsto #3]}
\newcommand{\subst}[3]{#3[#1/#2]}
\newcommand{\parsub}[1]{[#1]}
\newcommand{\dom}[1]{\mathrm{dom}(#1)}
\newcommand{\der}{\vdash}
\newcommand{\lolli}{\multimap}

% semantics
\newcommand{\dent}[1]{⟦#1⟧_{\category {Set}}}
\newcommand{\dentt}[2]{\dent{#1}_{#2}}
%% for palatino
%\def\lv{\mathopen{[\kern-0.2em[}}    % opening [[ value delimiter
%\def\rv{\mathclose{]\kern-0.2em]}}   % closing ]] value delimiter
% for computer modern
\def\lv{\mathopen{{[\kern-0.14em[}}}    % opening [[ value delimiter
\def\rv{\mathclose{{]\kern-0.14em]}}}   % closing ]] value delimiter
\newcommand{\den}[1]{⟦#1⟧_{\category {Set}}}
\newcommand{\Den}[3]{\den{#1}_{#2;#3}}
% \newcommand{\A}{\mathcal{A}}
% \newcommand{\B}{\mathcal{B}}
\newcommand{\R}{\mathrel{\RR}}
\newcommand{\RR}{\mathcal{R}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\Rel}{\mathsf{Rel}}
\newcommand{\WRel}{\mathsf{WRel}}
\newcommand{\Pot}{\mathcal{P}} % powerset
\newcommand{\op}{\mathsf{op}}
\newcommand{\Rop}{\mathrel{\RR^{\op}}}

\newcommand{\tzero}{\mathsf{zero}}
\newcommand{\tnil}{\mathsf{nil}}
\newcommand{\twrap}{\mathsf{wrap}}
\newcommand{\tunwrap}{\mathsf{unwrap}}
\newcommand{\Wrap}{\mathsf{Wrap}}
\newcommand{\tid}{\mathsf{id}}
\newcommand{\tswap}{\mathsf{swap}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\tList}{\mathsf{List}}
\newcommand{\List}{\tList\,}

%\newcommand{\implies}{\Longrightarrow}

\newcommand{\Ge}{\varepsilon}
\newcommand{\bu}{\bullet}
\newcommand{\Bang}[2][]{\mathrm{!}^{#2}_{#1}}
\newcommand{\curry}[1]{\mathsf{curry}(#1)}
\newcommand\appl{\mathsf{app}}
\newcommand{\uncurry}{\mathsf{uncurry}}

%% Categorical constructions (Not Syntax ™)
\newcommand\cobj[1]{\mathcolor{blue}{#1}}

\newcommand{\oand}{\cobj{\owedge}} %OR: \varowedge % LOOKS THE SAME.
\newcommand{\otop}{\cobj{\circled{\ensuremath{\scriptstyle\top}}}}
% \newcommand\withObj{\mathbin{∧\kern-1.1ex∧}}
\newcommand\withObj{\cobj{\With}}
\newcommand\topObj{\cobj{\Ttop}}
\newcommand\funObj{\cobj{\funOp}}
\newcommand\tensorObj{\cobj{\Tensor}}
\newcommand\unitObj{\cobj{1}}
\newcommand\sumObj{\cobj{⊕}}
\newcommand\KObj{\cobj{K}}
\renewcommand\hom{\to}
\newcommand\homBidir{↔}
\newcommand{\nf}{\ensuremath{\mathit{nf}}}

\input{core_macros.tex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-semantics"
%%% End:

